Astrophysical Objects in Modified Theories of Gravity

This thesis investigates compact astrophysical objects within modified theories of gravity, focusing on neutron stars and strange stars. The work studies their internal structure, equilibrium, and stability in gravitational frameworks based on torsion and nonmetricity, which provide the foundation for theories such as f(Q) and f(T) gravity. Charged isotropic compact star models are constructed in f(Q) gravity using conformal symmetry and the MIT Bag equation of state, with matching to the Bardeen exterior spacetime. Gravitational decoupling techniques, including minimal and complete geometric deformation methods, are employed in f(T) gravity to generate anisotropic strange star models. These approaches enable the inclusion of additional gravitational sources, dark matter effects, and spacetime deformations. Exact analytical solutions are obtained under suitable physical conditions such as regularity and vanishing complexity. The models are examined using energy conditions, causality constraints, the generalized Tolman-Oppenheimer-Volkoff equation, and Herrera's cracking criterion to ensure physical viability and stability. The influence of modified gravity parameters on stellar mass, radius, compactness, and stability is analyzed in detail. A Bayesian statistical framework is applied to constrain model parameters using observational data, including NICER mass-radius measurements. Bayes factor analysis is further used to identify viable gravitational extensions consistent with astrophysical observations. The results show that modified gravity can significantly affect the maximum mass, radius, and stability of compact stars while remaining compatible with observations. This work provides a systematic theoretical and observational study of compact stars beyond general relativity.

==> 1References.tex <==
\begin{thebibliography}{100}

%Chapter-1
\bibitem{Oppenheimer/1939} J. R. Oppenheimer, H. Snyder, \textit{Phys. Rev.} \textbf{56}, 455-459 (1939).
\bibitem{Eddington/1920} F.W. Dyson, A.S. Eddington, C.R. Davidson, \textit{Phil. Trans. Roy. Soc. A} \textbf{220}, 291333 (1920).
\bibitem{Damour/1999} T. Damour, \textit{Einsteins Path}, Springer New York, 171-187 (1999).
\bibitem{Schwarzschild/1916a} K. Schwarzschild, \textit{Sitzungsber. Preuss. Akad. D. Wiss. Berlin (Math.Phys.)} \textbf{1916}, 189-196 (1916).
\bibitem{Schwarzschild/1916b} K. Schwarzschild, \textit{Sitzungsber. Preuss. Akad. D. Wiss. Berlin (Math.Phys.)} \textbf{1916}, 424-434 (1916).
\bibitem{Reissner/1916} H. Reissner, \textit{Annalen der Physik} \textbf{355} (9), 106120 (1916).
\bibitem{Nordstrom/1918} G. Nordstrom, \textit{Verhandl. Koninkl. Ned. Akad. Wetenschap.} \textbf{26}, 12381245 (1918).



\bibitem{p1} A. G. Riess et al., \textit{Astron. J.} \textbf{116}, 1009 (1998).

\bibitem{p2} S. Perlmutter et al., \textit{Astrophys. J.} \textbf{517}, 565 (1999).

\bibitem{p3} N. Aghanim et al. (Planck Collaboration), \textit{Astron. Astrophys.} \textbf{641}, A6 (2020).

\bibitem{p4} T. Clifton, P. G. Ferreira, A. Padilla and C. Skordis, \textit{Phys. Rept.} \textbf{513}, 1 (2012).

\bibitem{p5} S. Nojiri and S. D. Odintsov, \textit{Phys. Rept.} \textbf{505}, 59 (2011).

\bibitem{p6} S. Capozziello and M. De Laurentis, \textit{Phys. Rept.} \textbf{509}, 167 (2011).


\bibitem{mass1}W.~M.~Farr, et al.,
\emph{APJ} \textbf{741}, 103 (2011).

\bibitem{mass2}F.~\"Ozel, et al., \emph{APJ} \textbf{725}, 1918 (2010).

\bibitem{torsion} K. Hayashi and T. Shirafuji
\textit{Phys. Rev. D} \textbf{19}, 3524 (1979).

\bibitem{nonmetricity} J. B. Jimenez, L. Heisenberg, T. Koivisto, \textit{Phys. Rev. D} \textbf{98}(4), 044048 (2018).
% \bibitem{dm50c} C. L. Bennett et al., \textit{Astrophys. J. (supp.)}, \textbf{148}, 97 (2003).
% \bibitem{dm51c} E. Komatsu et al., \textit{Astrophys. J. (supp.)} \textbf{180}, 330 (2009).
% \bibitem{dm52c} M. Tegmark et al., \textit{Phys. Rev. D} \textbf{74}, 123507 (2006).
% \bibitem{dm53c} W. J. Percival et al., \textit{MNRAS} \textbf{381}, 1053 (2007).
% \bibitem{dm54c} E. Aubourg et al., \textit{Phys. Rev. D} \textbf{92}, 123516 (2015).
% \bibitem{dm55c} A. Cooray and R. Sheth, \textit{Phys. Reports} \textbf{372}, 1-129 (2002).
% \bibitem{dm56c} G. L. Bryan and M. L. Norman \textit{Astrophys. J.} \textbf{495}, 80-99 (1998).
% \bibitem{dm57c} A. F. Neto et al., \textit{MNRAS} \textbf{381}, 1450 (2007).
% \bibitem{dm58c} A. A. Dutton and A. V. Maccio, \textit{MNRAS} \textbf{441}, 3359 (2014).
% \bibitem{dm59c} A. D. Ludlow et al., \textit{MNRAS} \textbf{441}, 378 (2014).
% %NFW DM
% \bibitem{dm50} J. Dubinski and R. G. Carlberg, \textit{Astrophys. J.} \textbf{378}, 496 (1991).
% \bibitem{dm51}  L. Hernquis, \textit{Astrophys. J.} \textbf{356}, 359 (1990).
% \bibitem{dm52} J. F. Navarro, C. S. Frenk, and S. D. M. White, \textit{Astrophys. J.} \textbf{462}, 563 (1996).
% \bibitem{dm53} J. F. Navarro, C. S. Frenk, and S. D. M. White, \textit{Astrophys. J.} \textbf{490}, 493 (1997).
% \bibitem{dm54} D. Merritt et al., \textit{Astrophys. J.} \textbf{132}, 2685 (2006).
% \bibitem{dm55} J. Stadel et al., \textit{MNRAS} \textbf{398}, L21 (2009).
% \bibitem{dm56} J. F. Navarro et al., \textit{MNRAS} \textbf{402}, 21 (2010).
% \bibitem{dm57} J. Einasto, \textit{Trudy Astrofizicheskogo Instituta Alma-Ata} \textbf{5}, 87 (1965).
% \bibitem{dm58} D. Merritt et al., \textit{Astrophys. J.} \textbf{132}, 2685 (2006).
% \bibitem{dm59} A. A. Dutton and A. V. Maccio, \textit{MNRAS} \textbf{441}, 3359 (2014).
% %BEC DM
% \bibitem{dm60} S. J. Sin, \textit{Phys. Rev. D} \textbf{50}, 3650 (1994). 
% \bibitem{dm61} S. U. Ji and S. J. Sin, \textit{Phys. Rev. D} \textbf{50}, 3655 (1994).
% \bibitem{dm62} W. Hu, R. Barkana, and A. Gruzinov, \textit{Phys. Rev. Lett.} \textbf{85}, 1158 (2000).
% \bibitem{dm63} S. Khlebnikov, \textit{Phys. Rev. A} \textbf{66}, 063606 (2002).
% \bibitem{dm64} M. Nishiyama, M. Morita, and M. Morikawa, 	arXiv: astro-ph/0403571 (2004).
% \bibitem{dm65} F. Ferrer and J. A. Grifols, \textit{J. Cosmo. Astro. Phys.} \textbf{0412}, 012 (2004).
% \bibitem{dm66} J. A. Grifols, \textit{Astropart. Phys.} \textbf{25}, 98 (2006).
% \bibitem{dm67} C. G. Boehmer and T. Harko, \textit{JCAP} \textbf{0706}, 025 (2007).
% \bibitem{dm68} F. Dalfovo, S. Giorgini, L. P. Pitaevskii, and S. Stringari, \textit{Rev. Mod. Phys.} \textbf{71}, 463 (1999).
% \bibitem{dm69} T. Harko, P. Liang, S. D. Liang, and G. Mocanu, \textit{JCAP} \textbf{1511}, 027 (2015).
% \bibitem{Begeman} K. G. Begeman, A. H. Broeils, and R. H. Sanders, \textit{MNRAS} \textbf{249}, 523 (1991).
% \bibitem{Frenk4} W. J. G. de Blok, Stacy S. McGaugh, Albert Bosma, and Vera C. Rubin, \textit{Astrophys. J.} \textbf{552}, L23-L26 (2001).
% \bibitem{pi1} G. Gentile, P. Salucci, U. Klein, D. Vergani, and P. Kalberla, \textit{MNRAS} \textbf{351}, 903 (2004).
% \bibitem{pi2} S-H. Oh, W. J. G. de Blok, E. Brinks, F. Walter, and R. C. Kennicutt Jr, \textit{Astrono. J.} \textbf{141}, 193 (2011).
% \bibitem{pi3} Z. Xu, M. Tang, G. Cao, and S.-N. Zhang, \textit{Eur. Phys. J. C} \textbf{80}, 70 (2020).
% \bibitem{dm70} A. Burkert, \textit{Astrophys. J.} \textbf{447}, L25-L28, (1995).
% \bibitem{dm71} J. F. Navarro, C. S. Frenk, and S. D. M. White, \textit{MNRAS} \textbf{275}, 720-740 (1995).
% \bibitem{dm72} M. Persic, P. Salucci, and F. Stel, \textit{MNRAS} \textbf{281}, 27 (1996).






% \bibitem{gr1}  T. P. Sotiriou, ``Modified Actions for Gravity: Theory and Phenomenology”, arXiv:gr-qc/0710.4438 (2007). 
% \bibitem{gr2} C. M. Will, ``Theory and Experiment in Gravitational Physics, revised edition", Cambridge University Press, Cambridge (1993).
% \bibitem{gr3} R. M. Wald, ``General Relativity", University of Chicago Press, United States of America (1984).
% \bibitem{gr4} A. Pais ``Subtle is the Lord: The Science and the Life of Albert Einstein”, Cambridge University Press (1982).
% \bibitem{gr5} W. Pauli, ``Theory of Relativity", Pergamon Press (1958).
% \bibitem{gr55} W. Rindler, ``Relativity: Special, General, and Cosmological", Second Edition, Oxford University Press (2006).
% \bibitem{gr6} K. S. Thorne and C. M. Will, \textit{Astrophys. J.} \textbf{163}, 595 (1971).
% \bibitem{gr7} V. A. Fock, ``The Theory of Space-Time and Gravitation", Pergamon Press, New York (1964).
% \bibitem{gr8} T. P. Sotiriou, V. Faraoni, and S. Liberati, \textit{Int. J. Mod. Phys. D} \textbf{17}, 399-423 (2008).
% \bibitem{otr1} R. D'Inverno, ``Introducing Einstein’s Relativity", Cambridge University Press, Cambridge (1998).
% % \bibitem{ot1} B. A. Dubrovin, A. T. Fomenko, and S. P. Novikov, ``Modern Geometry-Methods and Applications: Part I: The Geometry of Surfaces, Transformation Groups, and Fields", Second Edition, New York: Springer Verlag (1984).
% % \bibitem{ot2} L. D. Landau and E. M. Lifshitz, ``The Classical Theory of Fields", Amsterdam: Butterworth-Heinemann (1994).
% \bibitem{sp1} R. d'Inverno, ``Introducing Einstein’s Relativity", Clarendon Press (1992).
% \bibitem{sp2} C. W. Misner, K. S. Thorne, and J. A. Wheeler, ``Gravitation", W. H. Freeman and Co., San Francisco (1973).
% \bibitem{sp3} H. A. Buchdahl, \textit{MNRAS} \textbf{150}, 1-8 (1970).
% \bibitem{sp4} T. P. Sotiriou, V. Faraoni, and S. Liberati,
% \textit{Int. J. Mod. Phys. D} \textbf{17}, 399-423 (2008).
% \bibitem{sp5} J. M. Nester and H.-J. Yo, \textit{Chin. J. Phys.} \textbf{37}, 113 (1999).
% \bibitem{sp6} J. B. Jimenez, L. Heisenberg, and T. S. Koivisto, \textit{Universe} \textbf{5}, 173 (2019).
% \bibitem{sp7} T. Padmanabhan, ``Theoretical Astrophysics: Volume 3, Galaxies and Cosmology", Theoretical Astrophysics Cambridge University Press (2000).
% \bibitem{sp8} V. Sahni and A. A. Starobinsky, \textit{Int. J. Mod. Phys. D} \textbf{9}, 373 (2000).
% \bibitem{Padmanabhan/2003}T. Padmanabhan, \textit{Phys. Rep.} \textbf{380}, 235 (2003).
% \bibitem{sp9} S. Weinberg, \textit{Rev. Mod. Phys.} \textbf{61}, 1-23 (1989).
% \bibitem{sp10} E. J. Copeland, M. Sami, and S. Tsujikawa, \textit{Int. J. Mod. Phys. D} \textbf{15}, 1753 (2006).
% \bibitem{sp11} L. Amendola and S. Tsujikawa, ``Dark Energy: Theory and Observations", Cambridge University Press (2015).
% \bibitem{sp12} L. Verde, T. Treu, and A. G. Riess, \textit{Nature Astron.} \textbf{3}, 891 (2019).
% \bibitem{sp13} A. G. Riess et al, \textit{Astrophys. J. Lett.} \textbf{934}, L7 (2022).
% \bibitem{sp14} E. Macaulay, I. K. Wehus, and H. K. Eriksen, \textit{Phys. Rev. Lett.} \textbf{111}, 161301 (2013).
% \bibitem{sp15} M. Asgari et al, (KiDS), \textit{Astron. Astrophys.} \textbf{645}, A104 (2021).
% \bibitem{sp16} E. Di Valentino \textit{et\,al.}, \textit{Class. Quant. Grav.} \textbf{38}, 153001 (2021),
% \bibitem{sp17}  S. Nojiri, S. D. Odintsov, and V. K. Oikonomou, \textit{Phys. Rept.} \textbf{692}, 1-104 (2017).

% \bibitem{mg1}  M. Ostrogradsky, \textit{Mem. Acad. St. Petersbourg} \textbf{6}, 385-517 (1850).
% \bibitem{mg2} Thomas P. Sotiriou and Valerio Faraoni, \textit{Rev. Mod. Phys.} \textbf{82}, 451-497 (2010).
% \bibitem{mg3} Th. Kaluza, \textit{Zum Unit atsproblem der Physik. Sitzungsber. Preuss. Akad. Wiss. Berlin} \textbf{1921}, 966-972 (1921).
% \bibitem{mg4} G. R. Dvali, Gregory Gabadadze, and Massimo Porrati, \textit{Phys. Lett. B} \textbf{485}, 208-214 (2000).
% \bibitem{mg5} Gabriel R. Bengochea and Rafael Ferraro, \textit{Phys. Rev. D} \textbf{79}, 124019 (2009).
% \bibitem{mg6} J. B. Jimenez, L. Heisenberg, and Tomi S. Koivisto, \textit{Universe} \textbf{5}, 173 (2019).
% \bibitem{mg7} T. Jacobson and D. Mattingly, \textit{Phys. Rev. D} \textbf{64}, 024028 (2001).
% \bibitem{mg8} S. Tsujikawa, \textit{Class. Quant. Grav.} \textbf{30}, 214003 (2013).
% \bibitem{mg9} M. Banados, \textit{Phys. Rev. D} \textbf{77}, 123534 (2008).








% \bibitem{sp18} R. P. Woodard, \textit{Lect. Notes Phys.} \textbf{720}, 403 (2007).
% \bibitem{sp19} A. A. Starobinsky, \textit{JETP Lett.} \textbf{86}, 157 (2007).
% \bibitem{sp20} A. A. Starobinsky, \textit{Phys. Lett. B} \textbf{91}, 99 (1980).
% \bibitem{sp21} Y. Akrami \textit{et\,al.} (Planck), \textit{Astron. Astrophys.} \textbf{641}, A10 (2020).
% \bibitem{sp22} W. Hu and I. Sawicki, \textit{Phys. Rev. D} \textbf{76}, 64004 (2007).
% \bibitem{sp23} S. Xavier, J. Mathew, and S. Shankaranarayanan, \textit{Class. Quant. Grav.} \textbf{37}, 225006 (2020).
% %STEGR
% \bibitem{fq0} Tomas Ortin, ``Gravity and strings", Cambridge Monographs on Mathematical Physics Cambridge Univ. Press (2004).
% \bibitem{fq00} James M. Nester and Hwei-Jang Yo, \textit{Chin. J. Phys.} \textbf{37}, 113 (1999).
% \bibitem{fq000} Muzaffer Adak, M. Kalay, and Ozcan Sert, \textit{Int. J. Mod. Phys. D} \textbf{15}, 619-634 (2006).
% \bibitem{fq1} J. B. Jimenez, L. Heisenberg, and T. Kovisto, \textit{Phys. Rev. D} \textbf{98}, 044048 (2018).
% \bibitem{fq11} Igor Mol, \textit{Adv. Appl. Clifford Algebras} \textbf{27}, 2607-2638 (2017).
% \bibitem{fqt}Y. Xu et al.,	Eur. Phys. J. C \textbf{79}, 708 (2019).
% \bibitem{fq2} Avik De, Tee-How Loo, and Emmanuel N. Saridakis, \textit{JCAP} \textbf{03}, 050 (2024).
% %4D EGB
% \bibitem{egb1} D. Glavan and C. Lin, \textit{Phys. Rev. Lett.} \textbf{124}, 081301 (2020).
% \bibitem{egb2} D. Lovelock, \textit{J. Math. Phys.} \textbf{12}, 498 (1971).
% \bibitem{egb3} D. Lovelock, \textit{J. Math. Phys.} \textbf{13}, 874 (1972).
% \bibitem{egb4} T. Padmanabhan and D. Kothawala, \textit{Phys. Rep.} \textbf{531}, 115-171 (2013).
% \bibitem{egb6} C. Lanczos, \textit{Z. Phys.} \textbf{73}, 147-168 (1932).
% \bibitem{egb7} C. Lanczos, \textit{Ann. Math.} \textbf{39}, 842-850 (1938).
% \bibitem{egb5}  S. Chern, \textit{Ann. Math.} \textbf{46}, 674-84 (1945).
% %%%%%%%%%%%%%%%%%%%% END INTRODUCTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%CHAPTER-2 REFERENCES***********************************

% \bibitem{Laurentis} S. Capozziello and M. De Laurentis, \textit{Phys. Rept.} \textbf{509}, 167 (2011).
% \bibitem{Krssak} M. Krssak, R. J. van den Hoogen, J. G. Pereira, C. G. B\"ohmer, and A. A. Coley, \textit{Class. Quant. Grav.} \textbf{36}, 183001 (2019).
% \bibitem{Nester} James M. Nester and  Hwei-Jang Yo, \textit{Chin. J. Phys.} \textbf{37}, 113 (1999).
% \bibitem{Kalay} M. Adak, M. Kalay, and O. Sert, \textit{Int. J. Mod. Phys.} \textbf{D15}, 619 (2006).
% \bibitem{Conroy} A. Conroy and T. Koivisto, \textit{Eur. Phys. J. C} \textbf{78}, 923 (2018).
% \bibitem{Jimenez} J. B. Jimenez, L. Heisenberg, and T. S. Koivisto, \textit{Phys. Rev. D} \textbf{98}, 044048 (2018).
% \bibitem{Soudi} I. Soudi, G. Farrugia, V. Gakis, J. L. Said, and E. N. Saridakis, \textit{Phys. Rev. D} \textbf{100}, 044008 (2019).
% \bibitem{Banos} R. Lazkoz, F. S. N. Lobo, M. O. Banos, and V. Salzano, \textit{Phys. Rev. D} \textbf{100}, 104027 (2019).
% \bibitem{Salzano} I. Ayuso, R. Lazkoz, and V. Salzano, \textit{Phys. Rev. D} \textbf{103}, 063505 (2021).
% \bibitem{Koivisto11} B. J. Barros, T. Barreiro, T. Koivisto, and N. J. Nunes, \textit{Phys. Dark Univ.} \textbf{30}, 100616 (2020).
% \bibitem{Anagnostopoulos} F. K. Anagnostopoulos, S. Basilakos, and E. N. Saridakis, \textit{Phys. Lett. B} \textbf{822}, 136634 (2021).
% \bibitem{Fell} F. D'Ambrosio, S. D. B. Fell, L. Heisenberg, and S. Kuhn \textit{Phys. Rev. D} \textbf{105}, 024042 (2022).
% \bibitem{Zhai} Rui-Hui Lin and Xiang-Hua Zhai, \textit{Phys. Rev. D} \textbf{103}, 124001 (2021).
% \bibitem{Wang2} W. Wang, H. Chen, and T. Katsuragawa, \textit{Phys. Rev. D} \textbf{105}, 024060 (2022).
% \bibitem{Calza} M. Calza and L. Sebastiani, \textit{Eur. Phys. J. C} \textbf{83}, 247 (2023).
% \bibitem{Moraes/2017} P. H. R. S. Moraes and P. K. Sahoo, \textit{Phys. Rev. D} \textbf{96}, 044038 (2017).
% \bibitem{Elizalde/2019} E. Elizalde and M. Khurshudyan, \textit{Int. J. Mod. Phys. D} \textbf{28}, 1950172 (2019).
% \bibitem{kimet/2018} Kimet Jusufi, \textit{Phys. Rev. D} \textbf{98}, 044016 (2018).
% \bibitem{Lobo/2005} F. S. N. Lobo, \textit{Phys. Rev. D} \textbf{71}, 084011 (2005).
% \bibitem{Francisco/2005} F. S. N. Lobo, \textit{Phys. Rev. D} \textbf{71}, 124022 (2005).
% \bibitem{Mauricio/2013} Mauricio Cataldo and Paola Meza, \textit{Phys. Rev. D} \textbf{87}, 064012 (2013).
% %\bibitem{Visser/2003} M. Visser, S. Kar, and N. Dadhich, \href{https://journals.aps.org/prl/abstract/10.1103/PhysRevLett.90.201102}{\prl \,\ \textbf{90}, 201102 (2003)}.
% \bibitem{Newton/2020} Ksh. Newton Singh, Ayan Banerjee, Farook Rahaman, and M. K. Jasim, \textit{Phys. Rev. D} \textbf{101}, 084012 (2020).
% \bibitem{Visser/2003} M. Visser, S. Kar, and N. Dadhich, \textit{Phys. Rev. Lett.} \textbf{90}, 201102 (2003).
% \bibitem{Jusufi/2020} K. Jusufi, A. Banerjee, and S. G. Ghosh, \textit{Eur. Phys. J. C} \textbf{80}, 698 (2020).
% % \bibitem{Hassan1} Zinnat Hassan, Sanjay Mandal, P.K. Sahoo, \textit{Forts. Phys.} \textbf{69}, 2100023 (2021).
% % \bibitem{Mustafa} G. Mustafa, Z. Hassan, P.H.R.S. Moraes, P.K. Sahoo, \textit{Phys. Lett. B} \textbf{821}, 136612 (2021).
% % \bibitem{1} M. Calza and L. Sebastiani, \textit{arXiv}, arXiv:2208.13033 [gr-qc].
% % \bibitem{Sokoliuk} O. Sokoliuk, Z. Hassan, P.K. Sahoo, A. Baransky, \textit{Ann. Phys.} \textbf{443}, 168968 (2022).
% % \bibitem{Sahoo111} G. Mustafa, Z. Hassan, P. K. Sahoo, \textit{Ann. Phys.} \textbf{437}, 168751 (2022).
% % \bibitem{Hassan3} S. Mandal, G. Mustafa, Z. Hassan, P. K. Sahoo \textit{Phys. Dark Univ.} \textbf{35}, 100934 (2022)


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%CHAPTER-3 REFERENCES*********(PLB paper)*****************************************

% % \bibitem{Jimenez/2018} J. B. Jim\'enez, L. Heisenberg, T. Koivisto, Phy. Rev. D, \textbf{98}, 044048 (2018).
% % \bibitem{maluf/2013} J. W. Maluf, \textit{Ann. Phys.} {\bf 525}, 339 (2013).
% % \bibitem{Ratanpal1} S.K. Maurya, B.S. Ratanpal, and M. Govender, \textit{Ann. Phys.} \textbf{382}, 36 (2017).
% % \bibitem{Ratanpal2} S. Gedela, R.K. Bisht, and N. Pant, Neeraj, \textit{Mod. Phys. Lett. A} \textbf{34}, 1950157 (2019).
% % \bibitem{Bhar1} P. Bhar, \textit{Eur. Phys. J. C} \textbf{79}, 138 (2019).
% % \bibitem{Bhar2} S. Gedela, R. K. Bisht, and N. Pant, \textit{Eur. Phys. J. A} \textbf{54}, 207 (2018).
% % %\bibitem{Bhar3} K. N. Singh, S. K. Maurya, and A. Errehymy, et al., \textit{Phys. Dark Univ.} \textbf{30}, 100620 (2020).
% % \bibitem{Hansraj} S. Hansraj and L. Moodly, \textit{Eur. Phys. J. C} \textbf{80}, 496 (2020).
% % \bibitem{Naidu1} N. F. Naidu, M. Govender, and S. D. Maharaj, \textit{Eur. Phys. J. C} \textbf{78}, 48 (2018).
% % \bibitem{Naidu2} J. Ospino and L. A. Nunez, \textit{Eur. Phys. J. C} \textbf{80}, 166 (2020).
% % \bibitem{Naidu3} S. C. Jaryal, \textit{Eur. Phys. J. C} \textbf{80}, 683 (2020).
% % \bibitem{Maurya4} S. K. Maurya, et al. \textit{Eur. Phys. J. C} \textbf{81}, 729 (2021).
% % \bibitem{Eiesland} J. Eiesland, \textit{Trans. Am. Math. Soc.} \textbf{27}, 213 (1925).
% % \bibitem{Eisenhart1} L. P. Eisenhart, \textit{Riemannian Geometry}, (Princeton University Press, Princeton, United States of America, 1966).
% % \bibitem{Karmarkar1} K. R. Karmarkar, \textit{Proc. Indian Acad. Sci. A} \textbf{27} 56 (1948).
% % \bibitem{Pandey1} S. N. Pandey and S. P. Sharma, \textit{Gen. Relativ. Gravit.} \textbf{14}, 113 (1981).
% % \bibitem{Gupta/1975} Y. K. Gupta, and M.P. Goel., \textit{Gen. Rel. Grav.} 6, 499 (1975).
% % \bibitem{Zia} M.F. Shamir and S. Zia, \textit{Astrophys. Space Sci.} \textbf{363}, 247 (2017).
% % \bibitem{Anchordoqui} L.A. Anchordoqui, D.F. Torres, M.L. Trobo, and S.E.P. Bergliaffa, \textit{Phys. Rev. D} \textbf{57}, 829 (1998).
% % \bibitem{Pavlovic/2015} P. Pavlovic, M. Sossich, \textit{Eur. Phys. J. C} \textbf{75}, 117 (2015).
% % \bibitem{Elizalde/2011} E. Elizalde, S. Nojiri, S.D. Odintsov, L. Sebastiani, S. Zerbini, \textit{Phys. Rev. D} \textbf{83}, 086006 (2011).
% % \bibitem{Tsujikawa/2008} S. Tsujikawa, \textit{Phys. Rev. D} \textbf{77}, 023507 (2008).

% % \bibitem{rahaman/2014} Farook Rahaman, P. K. F. Kuhfittig, Saibal Ray, and Nasarul Islam, {\it Eur. Phys. J. C} {\bf 74}, 2750 (2014).
% % \bibitem{ovgun/2016} A. {\" O}vg{\" u}n and M. Halilsoy, {\it Astrophys. Spa. Sci.} {\bf 361}, 214 (2016).
% % \bibitem{safonova/2002} Margarita Safonova, Diego F. Torres, and Gustavo E. Romero, {\it Phys. Rev. D} {\bf 65}, 023001 (2001).
% % \bibitem{bambi/2021} C. Bambi and D. Stojkovic, arXiv:2105.00881.

% % \bibitem{dai/2019} D.-C. Dai and D. Stojkovic, Phys. Rev. D {\bf 100}, 083513 (2019).
% % \bibitem{cramer/1995} J.G. Cramer et al., Phys. Rev. D {\bf 51}, 3117 (1995).
% % \bibitem{wang/2020} X. Wang et al., Phys. Lett. B {\bf 811}, 135930 (2020).
% % \bibitem{ohgami/2015} T. Ohgami and N. Sakai, Phys. Rev. D {\bf 91}, 124020 (2015).
% % \bibitem{torres/1998} D.F. Torres et al., Phys. Rev. D {\bf 58}, 123001 (1998).
% % \bibitem{shaikh/2018} R. Shaikh, Phys. Rev. D {\bf 98}, 024044 (2018).
% % \bibitem{nandi/2006} K.K. Nandi et al., Phys. Rev. D {\bf 74}, 024020 (2006).
% % \bibitem{jusufi/2018} K. Jusufi and A. \~A-vg\"{u}n, Phys. Rev. D {\bf 97}, 024042 (2018).
% % \bibitem{damour/2007} T. Damour and S.N. Solodukhin, Phys. Rev. D {\bf 76}, 024016 (2007).
% % \bibitem{Morris} M. S. Morris and K. S. Thorne, \textit{Am. J. Phys.} \textbf{56}, 395 (1988).
% % \bibitem{hawking/1973} S.W. Hawking and G.F.R. Ellis, The Large Scale Structure of Space-Time (Cambridge University Press, Cambridge, England, 1973).
% % \bibitem{visser/1995} M. Visser, Lorentzian Wormholes: from Einstein to Hawking (AIP Press, New York, United States of America, 1995).

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%CHAPTER-3 (GRG paper) REFERENCES***************************************************
% \bibitem{casimir}  H. B. G. Casimir,  D. Polder, \textit{Phys. Rev.} \textbf{73}, 360-372 (1948).
% \bibitem{lifshitz} I. E. Dzyaloshinskii, E. M. Lifshitz, and Lev P Pitaevskii,  \textit{Soviet Physics Uspekhi.} \textbf{4}, 153 (1961).
% \bibitem{experiment} S. K. Lamoreaux, \textit{ Phys. Rev. Lett.} \textbf{78}, 5-8 (1997).
% \bibitem{bressi} G. Bressi, G. Carugno, R. Onofrio, and G. Ruoso, \textit{Phys. Rev. Lett.} \textbf{88}, 041804 (2002).
% \bibitem{Garattini} R. Garattini, \textit{Eur. Phys. J. C} \textbf{79}, 951 (2019).
% \bibitem{rainbowsmolin}  J. Magueijo and L. Smolin, \textit{Class. Quant. Grav.} \textbf{21}, 1725 (2004).
% %\bibitem{sabinegup} S. Hossenfelder 
% %\textit{Living Rev. Relativity},\textbf{16}, 2, (2013).
% \bibitem{7} R. Garattini, \textit{Eur. Phys. J. C} \textbf{79}, 951 (2019).
% \bibitem{Channuie} D. Samart, T. Tangphati, and P. Channuie, \textit{Nucl. Phys. B} \textbf{980}, 115848 (2022).

% \bibitem{g1} M. Adak, O. Sert, M. Kalay, and M. Sari, \textit{Int. J. Mod. Phys. A} \textbf{28}, 1350167 (2013). 
% \bibitem{g2} M. Adak, M. Kalay, and O. Sert, \textit{Int. J. Mod. Phys. D} \textbf{15}, 619 (2006).
% \bibitem{g3} I. Mol, \textit{Adv. Appl. Clifford Algebras} \textbf{27}, 2607 (2017).
% \bibitem{g4} M. Krssak and E. N. Saridakis, \textit{Class. Quant. Grav.} \textbf{33}, 115009 (2016).
% \bibitem{rk} Rui-Hui Lin and Xiang-Hua Zhai, \textit{Phys. Rev. D} \textbf{103}, 124001 (2021).
% \bibitem{zee} A. Zee, ``Quantum Field Theory in a Nutshell", Second Edition, Princeton University Press (2010).
% \bibitem{paddy} T. Padmanabhan, ``Quantum Field Theory The Why, What and How", First Edition, Springer (2016).
% \bibitem{Bezerra} G. Alencar, V. B. Bezerra, and C. R. Muniz, \textit{Eur. Phys. J. C} \textbf{81}, 924 (2021).
% \bibitem{Fuenmayor} R. Avalos, E. Fuenmayor, and E. Contreras, \textit{Eur. Phys. J. C} \textbf{82}, 420 (2022).
% \bibitem{Khabibullin} A. R. Khabibullin et al., \textit{Class. Quant. Grav.} \textbf{23}, 627 (2006).
% %\bibitem{gupcasimir} A. M. Frassino, O. Panella, \textit{Phys. Rev. D}  \textbf{85} 045030 (2012).
% \bibitem{Solanki} R. Solanki, A. De, and P. K. Sahoo, \textit{Phys. Dark Univ.} \textbf{36}, 101053 (2022).
% \bibitem{Parbati} P. Sahoo, A. De, Tee-How Loo, and P. K. Sahoo, \textit{Comm. Theor. Phys.} \textbf{74}, 125402 (2022).
% \bibitem{Kazuharu} Z. Hassan, S. Ghosh, P. K. Sahoo, and K. Bamba, \textit{Eur. Phys. J. C} \textbf{82}, 1116 (2022).
% \bibitem{Visser} M. Visser, ``Lorentzian Wormholes: From Einstein to Hawking", First Edition, American Institute of Physics, New York
% (1996).
% \bibitem{Pradhan} A. Banerjee, A. Pradhan, T. Tangphati, and F. Rahaman, \textit{Eur. Phys. J. C} \textbf{81}, 1031 (2021).
% % \bibitem{adm0} R. M. Wald, \textit{General Relativity} (University of Chicago Press, Chicago, 1984).
% % \bibitem{adm1} R. Shaikh, \textit{Phys. Rev. D} \textbf{98}, 024044 (2018).
% % \bibitem{adm2} P. T. Chrusciel, Lectures on Energy in General Relativity, Krakow, 2010.
% %\bibitem{Visser3} M. Visser, S. Kar and N. Dadhich, \textit{Phys. Rev. Lett.} \textbf{90}, 201102 (2003).
% \bibitem{Channuie1} K. Jusufi, P. Channuie, and M. Jamil, \textit{Eur. Phys. J. C} \textbf{80}, 127 (2020).
% \bibitem{Baransky} O. Sokoliuk, S. Mandal, P. K. Sahoo, and A. Baransky, \textit{Eur. Phys. J. C} \textbf{82}, 280 (2022).
% % \bibitem{rainbowsmolin}  J. Magueijo, L. Smolin \textit{Class. Quantum Grav.} \textbf{21} 1725 (2004).
% % \bibitem{sabinegup} S. Hossenfelder 
% % \textit{Living Rev. Relativity},\textbf{16}, 2, (2013).
% \bibitem{regula} A. Kempf and G. Mangano  \textit{Phys. Rev. D} \textbf{55}, 7909 (1997).
% \bibitem{Tripathy} S. K. Tripathy, \textit{Phys. Dark Univ.} \textbf{31}, 100757 (2021).
% %\bibitem{Koivisto} J. B. Jimenez, L. Heisenberg, T. Koivisto, and S. Pekar, \textit{Phys. Rev. D} \textbf{101}, 103507 (2020).
% \bibitem{qedgup1} O. Panella, \textit{Phys. Rev. D} \textbf{76}, 045012 (2007).
% \bibitem{qedgup2} K. Nouicer, \textit{J. Phys. A} \textbf{38}, 10027 (2005).

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%CHAPTER-4 (CQG paper)*************************************************

% \bibitem{Rubin1} V. C. Rubin, W. K. Jr. Ford, and  N. Thonnard, \textit{Astrophys. J.} \textbf{238}, 471-487 (1980).
% \bibitem{Rubin2} F. Zwicky, \textit{Gen. Rel. Grav.} \textbf{41}, 207-224 (2009).
% \bibitem{Rubin3} P. A. R. Ade et al., \textit{Astron. Astrophys.} \textbf{594}, A13 (2016).
% \bibitem{Rahaman1} F. Rahaman, P. K. F. Kuhfittig, S. Ray, and N. Islam, \textit{Eur. Phys. J. C} \textbf{74}, 2750 (2014).
% \bibitem{Rahaman2} F. Rahaman, P. Salucci,  K. F. Kuhfittig, S. Ray, and  M. Rahaman, \textit{Ann. Phys.} \textbf{350}, 561 (2014).
% \bibitem{Rahaman3} J. F. Navarro, C. S. Frenk, and S. D. M. White,  \textit{Astrophys. J.} \textbf{462}, 563 (1996).
% \bibitem{Rahaman4} F. Rahaman, G. C. Shit, B. Sen, and S. Ray, \textit{Astrophys. Space Sci.} \textbf{361}, 37 (2016).
% \bibitem{Rahaman6} S. Islam, F. Rahaman, A. Ovgun, and M. Halilsoy,  \textit{Can. J. Phys.} \textbf{97}, 241 (2019).
% \bibitem{Rahaman5} P. Salucci and Ch. Frigerio Martins, \textit{EAS Publ. Ser.} \textbf{36}, 133 (2009).
% \bibitem{Jusufi1} K. Jusufi, M. Jamil, and M. Rizwan, \textit{Gen. Rel. Grav.} \textbf{51}, 102 (2019).
% \bibitem{Jusufi2} J. Einasto and U. Haud, \textit{Galaxy Astron. Astrophys.} \textbf{223}, 89 (1989).
% \bibitem{Jusufi3} K. G. Begeman, A. H. Broeils, and R. H. Sanders, \textit{MNRAS} \textbf{249}, 523 (1991).
% \bibitem{Milgrom1} M. Milgrom, \textit{Phys. Rev. Lett.} \textbf{117}, 141101 (2016).
% \bibitem{Milgrom2} M. Milgrom, \textit{Astrophys. J.} \textbf{270}, 365 (1983).
% \bibitem{Milgrom3} M. Milgrom, \textit{Astrophys. J.} \textbf{270}, 371 (1983).
% \bibitem{Milgrom4} B. C. Paul, \textit{Class. Quant. Grav.} \textbf{38}, 145022 (2021).
% \bibitem{sd1} J. L. Synge, \textit{MNRAS} \textbf{131}, 463 (1966).
% \bibitem{sd2} J. P. Luminet, \textit{Astron. Astrophys.} \textbf{75}, 228 (1979).
% \bibitem{sd3} H. Falcke, F. Melia, and E. Agol, \textit{Astrophys.  J.} \textbf{528}, L13 (2000).
% %\bibitem{sd4} V. Perlick and O. Y. Tsupko, \textit{Phys. Rep.} \textbf{947}, 1 (2022).
% \bibitem{sd5} K.  Akiyama et al., \textit{Astrophys.  J.} \textbf{875}, L1 (2019).
% \bibitem{sd6} K. Akiyama et al., \textit{Astrophys. J. Lett} \textbf{930}, L12 (2022).
% \bibitem{sd7} C. Bambi and K. Freese, \textit{Phys. Rev. D.} \textbf{79}, 043002 (2009).
% \bibitem{sd8} A. Abdujabbarov et al., \textit{Phys. Rev. D} \textbf{93}, 104004 (2016).
% \bibitem{sd9} X. Hou,  Z. Xu,  and  J. Wang, \textit{J.  Cosmo.  Astro.  Phys.} \textbf{2018}, 040 (2018).
% \bibitem{sd10} P. V. P. Cunha, N. A. Eiro, C. A. R. Herdeiro, and J. P. S. Lemos, \textit{J.  Cosmo.  Astro.  Phys.} \textbf{2020}, 035 (2020).
% \bibitem{sd11} M.  Afrin,  R.  Kumar,  and  S.  G.  Ghosh, \textit{MNRAS} \textbf{504}, 5927 (2020).
% % \bibitem{sd12} F.  Atamurotov,  U.  Papnoi,  and  K.  Jusufi, \textit{Class. Quant. Grav.} \textbf{39}, 025014 (2022).
% % \bibitem{sd13} X. Wang, P.-C. Li, C.-Y. Zhang, and M. Guo, \textit{Phys. Lett. B} \textbf{811}, 135930 (2020).
% % \bibitem{sd14} V. Perlick  and  O. Y. Tsupko, \textit{Phys. Rep.} \textbf{947}, 1 (2022).
% % \bibitem{sd15} M. Alloqulov et al., \textit{Chinese Phys. C} \textbf{48}, 025104 (2024).
% \bibitem{Einstein10} A. Einstein, \textit{Science} \textbf{84}, 506 (1936).
% \bibitem{Dyson} F. W. Dyson, A. S. Eddington, and C. Davidson, \textit{Philos. Trans. R. Soc. A} \textbf{220}, 291 (1920).
% \bibitem{Eddington} A. S. Eddington, ``Space, Time and Gravitation", Cambridge University Press, Cambridge, England (1920).
% \bibitem{Sahu} K. C. Sahu et al., \textit{Science} \textbf{356}, 1046 (2017).
% \bibitem{Bozza1} V. Bozza, S. Capozziello, G. Iovane, and G. Scarpetta , \textit{Gen. Rel. Grav.} \textbf{33}, 1535-1548 (2001).
% \bibitem{Virbhadra} K. S. Virbhadra and G. F. R. Ellis, \textit{Phys. Rev. D} \textbf{62}, 084003 (2000).
% \bibitem{Bozza22} V. Bozza, \textit{Phys. Rev. D} \textbf{66}, 103001 (2002).
% \bibitem{A1}  N. Tsukamoto,  \textit{Phys. Rev. D} \textbf{94}, 124001 (2016).
% \bibitem{A2} Y. Kumaran and A. Ovgun, \textit{Turk. J. Phys.} \textbf{45}, 247-267 (2021).
% \bibitem{A3} A. Ovgun, \textit{Turk. J. Phys.} \textbf{44}, 465-471 (2020).
% \bibitem{A4} W. Javed, R. Babar, and A. Ovgun, \textit{Phys. Rev. D} \textbf{99}, 084012 (2019).
% % \bibitem{A5} R. Shaikh and S. Kar, \textit{Phys. Rev. D} \textbf{96}, 044037 (2017).
% % \bibitem{A6} A. Ovgun, \textit{Phys. Rev. D} \textbf{98}, 044033 (2018).
% % \bibitem{A7} K. Jusufi and A. Ovgun, \textit{Phys. Rev. D} \textbf{97}, 024042 (2018).
% % \bibitem{A8} W. Javed et al, \textit{Eur. Phys. J. C} \textbf{82}, 1057 (2022).
% % \bibitem{A9}  S. N. Sajadi and N. Riazi, \textit{Can. J. Phys.} \textbf{98}, 1046-1054 (2020).
% % \bibitem{A10} W. Javed et al., \textit{Universe} \textbf{8}, 599 (2022).
% \bibitem{dz1} R. Ferraro and F. Fiorini, \textit{Phys. Rev. D} \textbf{84}, 083518 (2011).
% \bibitem{dz2} W. Wang, H. Chen, and T. Katsuragawa,  \textit{Phys. Rev. D} \textbf{105}, 024060 (2022).
% \bibitem{dz3} D. Zhao, \textit{Eur. Phys. J. C} \textbf{82}, 303 (2022).
% \bibitem{Hawking} S. W. Hawking and G. F. R. Ellis, ``The Large Scale Structure of Space-Time", Cambridge University Press, England (1973).
% \bibitem{Raychaudhuri} A. Raychaudhuri, \textit{Phys. Rev.} \textbf{98}, 1123 (1955).
% \bibitem{ws1} J. M. Bardeen, W. H. Press, and S. A. Teukolsky, \textit{Astrophys. J.} \textbf{178}, 347 (1972).
% \bibitem{ws2} K. Hioki and K.-ichi Maeda, \textit{Phys. Rev. D} \textbf{80}, 024042 (2009).
% \bibitem{ws3} S. E. Vazquez and E. P. Esteban, \textit{Nuovo Cimento B Serie} \textbf{119}, 489 (2004).
% \bibitem{ws4} P. G. Nedkova, V. Tinchev, and S. S. Yazadjiev,
% \textit{Phys. Rev. D} \textbf{88}, 124019 (2013).
% \bibitem{Virbhadra1} K. S. Virbhadra, D. Narasimha, and S. M. Chitre, \textit{Astron. Astrophys.} \textbf{337}, 1 (1998).
% %\bibitem{Virbhadra2} K. S. Virbhadra and G. F. R. Ellis, \textit{Phys. Rev. D} \textbf{62}, 084003 (2000).
% \bibitem{Virbhadra3} C. M. Claudel, K. S. Virbhadra, and G. F. R. Ellis, \textit{J. Math. Phys.} \textbf{42}, 818 (2001).
% %\bibitem{Bozza2} V. Bozza, \textit{Phys. Rev. D} \textbf{66}, 103001 (2002).
% \bibitem{Quinet} J. P. S. Lemos, F. S. N. Lobo, and S. Quinet de Oliveira, \textit{Phys. Rev. D} \textbf{68}, 064004 (2003).
% \bibitem{Tejeiro} J. M. Tejeiro and E. A. Larranaga, \textit{Rom. J. Phys.} \textbf{57}, 736 (2012).
% %\bibitem{g11} R. Shaikh, P. Banerjee, S. Paul, and T. Sarkar, \textit{JCAP} \textbf{07}, 028 (2019).
% \bibitem{r4} N. Godani and G. C. Samanta, \textit{Ann. Phys.} \textbf{429}, 168460 (2021).
% \bibitem{r1} R. Shaikh, P. Banerjee, S. Paul, and T. Sarkar, \textit{Phys. Lett. B} \textbf{789}, 270-275 (2019).
% \bibitem{r2} D. Samart, N. Autthisin, and P. Channuie, \textit{Anna. Physik} \textbf{535}, 2300039 (2023).
% \bibitem{r3} P. K. F. Kuhfittig, \textit{Eur. Phys. J. C} \textbf{74}, 2818 (2014).
% \bibitem{c1} F. Rahaman, G. C. Shit, B. Sen, and S. Ray, \textit{Astrophys. Space Sci.} \textbf{361}, 37 (2016).
% \bibitem{c2} F. Rahaman et al. \textit{Ann. Phys.} \textbf{350}, 561 (2014).
% %\bibitem{c3} K. Jusufi, M. Jamil, and M. Rizwan, \textit{Gen. Rel. Grav.} \textbf{51}, 102 (2019).
% \bibitem{c4} G. Mustafa, F. Atamurotov, and S. G. Ghosh, \textit{Phys. Dark Univ.} \textbf{40}, 101214 (2023).

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%CHAPTER-5 (ADP paper) REFERENCES***************************************************

% \bibitem{Zwiebach1} B. Zwiebach, \textit{Phys. Lett. B} \textbf{156}, 315 (1985).
% %\bibitem{Zwiebach2} M. J. Duff, B. E. W. Nilsson, and C. N. Pope, \textit{Phys. Lett. B} \textbf{173}, 69 (1986).
% \bibitem{Zwiebach3} D. J. Gross and J. H. Sloan, \textit{Nucl. Phys. B} \textbf{291}, 41 (1987).
% \bibitem{Zwiebach4} M.C. Bento and O. Bertolami, \textit{Phys. Lett. B} \textbf{368}, 198 (1996).
% %\bibitem{Lanczos} C. Lanczos, \textit{Ann. Math.} \textbf{39}, 842 (1938).
% \bibitem{Lovelock1} D. Lovelock, \textit{J. Math. Phys.} \textbf{12}, 498 (1971).
% \bibitem{Lovelock2} D. G. Boulware and S. Deser, \textit{Phys. Rev. Lett.} \textbf{55}, 2656 (1985).
% % \bibitem{Lovelock3} J. T. Wheeler, \textit{Nucl. Phys. B} \textbf{268}, 737 (1986).
% % \bibitem{Lovelock4} F. R. Tangherlini, \textit{Nuovo Cim.} \textbf{27}, 636 (1963).

% \bibitem{Lin1} D. Glavan and C. Lin, \textit{Phys. Rev. Lett.} \textbf{124}, 081301 (2020).
% \bibitem{Aoki1} K. Aoki, M.A. Gorji, and S. Mukohyama, \textit{Phys. Lett. B} \textbf{810}, 135843 (2020).
% \bibitem{Aoki2} K. Aoki, M.A. Gorji, and S. Mukohyama, \textit{J. Cosmo. Astro. Phys.} \textbf{2009}, 014 (2020).


% \bibitem{Lin2} R. A. Konoplya and A. Zhidenko, \textit{Phys. Dark Univ.} \textbf{30}, 100697 (2020).
% %\bibitem{Lin3} K. Hegde et al., \textit{arXiv} arXiv:2003.08778
% \bibitem{Lin4} C.-Y. Zhang, P.-C. Li, and M. Guo, \textit{Eur. Phys. J. C} \textbf{80}, 874 (2020).
% \bibitem{Lin5} H. Lu and Y. Pang, \textit{Phys. Lett. B} \textbf{809}, 135717 (2020).
% \bibitem{Lin6} M. S. Churilova, \textit{Phys. Dark Univ.} \textbf{31}, 100748 (2021).
% %\bibitem{Lin7} P. G. S. Fernandes, \textit{Phys. Lett. B} \textbf{805}, 135468 (2020).
% \bibitem{Lin8} D. V. Singh, S. G. Ghosh and S. D. Maharaj, \textit{Phys. Dark Univ.} \textbf{30}, 100730 (2020).
% \bibitem{Lin9} S. G. Ghosh and R. Kumar, \textit{Class. Quant. Grav.} \textbf{37}, 245008 (2020).
% \bibitem{Doneva1} D. D. Doneva and S. S. Yazadjiev, \textit{J. Cosmo. Astro. Phys.} \textbf{2021}, 024 (2021).
% \bibitem{Doneva2} R. A. Konoplya and A. Zhidenko, \textit{Phys. Rev. D} \textbf{102}, 064004 (2020).
% \bibitem{Doneva3} S.-W. Wei and Y.-X. Liu, \textit{Eur. Phys. J. Plus} \textbf{136}, 436 (2021).
% % \bibitem{Doneva4} R. Kumar and S. G. Ghosh, \textit{J. Cosmo. Astro. Phys.} \textbf{2020}, 053 (2020).
% % \bibitem{Doneva5} S. A. Hosseini Mansoori, \textit{Phys. Dark Univ.} \textbf{31}, 100776 (2021).
% \bibitem{Guo} M. Guo and P.-C. Li, \textit{Eur. Phys. J. C} \textbf{80}, 588 (2020).
% \bibitem{Mulryne} P. G. S. Fernandes, P. Carrilho, T. Clifton, and D. J. Mulryne, \textit{Class. Quantum Grav.} \textbf{39}, 063001 (2022).

% % \bibitem{Sisman} M. Gurses, T. C. Sisman, and B. Tekin, \textit{Eur. Phys. J. C} \textbf{80}, 647 (2020).
% % \bibitem{Carrilho1} Pedro G. S. Fernandes, P. Carrilho, T. Clifton, and D. J. Mulryne, \textit{Phys. Rev. D} \textbf{102}, 024025 (2020).
% % \bibitem{Carrilho2} R. A. Hennigar, D. Kubiznak, R. B. Mann, and C. Pollack, \textit{J. High Energ. Phys.} \textbf{2020}, 27 (2020).
% % \bibitem{Ai1} Wen Yuan Ai, \textit{Commun. Theor. Phys.} \textbf{72}, 095402 (2020).
% % \bibitem{Ai2} Fu-Wen Shu, \textit{Phys. Lett. B} \textbf{811}, 135907 (2020).
% % \bibitem{Ai3} S. Mahapatra, \textit{Eur. Phys. J. C} \textbf{80}, 992 (2020).
% % \bibitem{Ai4} J. Arrechea et al. \textit{Chinese Phys. C} \textbf{45} 013107 (2021).
% % \bibitem{Kobayashi1} T. Kobayashi, \textit{J. Cosmo. Astro. Phys.} \textbf{2020}, 013 (2020).
% % \bibitem{Kobayashi2} H. Lu and Yi Pang, \textit{Phys. Lett. B} \textbf{809}, 135717 (2020).
% % \bibitem{Kobayashi3} A. Casalino, A. Colleaux, M. Rinaldi, and S. Vicentini, \textit{Phys. Dark. Univ.} \textbf{31}, 100770 (2021).
% % \bibitem{Kobayashi4} L. Ma and H. Lu, \textit{Eur. Phys. J. C} \textbf{80}, 1209 (2020).

% \bibitem{Jusufi11} K. Jusufi, A. Banerjee, and S. G. Ghosh, \textit{Eur. Phys. J. C} \textbf{80}, 698 (2020).
% \bibitem{Jusufi22} N. Godani, D. V. Singh, G. C. Samanta, \textit{Phys. Dark Univ.} \textbf{35}, 100952 (2022).
% \bibitem{Jusufi33} Shweta, U. K. Sharma, and A. K. Mishra, \textit{Int. J. Geo. Mod. Phys.} \textbf{20} 2350140 (2023).
% \bibitem{Zwicky1} F. Zwicky, \textit{Helv. Phys. Acta} \textbf{6}, 110 (1933)
% \bibitem{Zwicky2} F. Zwicky, \textit{Astrophys. J.} \textbf{86}, 217 (1937).
% \bibitem{Oort1} J. Oort, \textit{Bull. Astron. Ins. Nether. V} \textbf{192} (1930).
% \bibitem{Oort2} J. Oort, \textit{Bull. Astron. Ins. Nether. V} \textbf{239} (1930).
% \bibitem{Diemand} J. Diemand et al., \textit{Nature} \textbf{454}, 735 (2008).
% \bibitem{Springel} V. Springel et al., \textit{MNRAS} \textbf{391}, 1685 (2008).
% %\bibitem{Pato} F. Iocco, M. Pato, G. Bertone, P. Jetzer, \textit{J. Cosmol. Astropart. Phys.} \textbf{2011}, 029 (2011).
% %\bibitem{Faber} T. Faber and M. Visser, \textit{MNRAS} \textbf{372}, 136 (2006).
% %\bibitem{Kalam} F. Rahaman, M. Kalam, A. DeBenedictis, A. Usmani, S. Ray, \textit{MNRAS} \textbf{389}, 27 (2008).
% %\bibitem{Filippov} K. K. Nandi, A. I. Filippov, F. Rahaman et al., \textit{MNRAS} 399, 2079 (2009).
% \bibitem{Rahaman66} F. Rahaman, G. C. Shit, B. Sen, S. Ray, \textit{Astrophys. Space Sci. }\textbf{361}, 37 (2016).
% \bibitem{Sarkar2} N. Sarkar, et al. \textit{Mod. Phys. Lett. A} \textbf{34}, 1950188 (2019).
% \bibitem{Rahaman8} P. K. F. Kuhfittig, \textit{Eur. Phys. J. C} \textbf{74}, 2818 (2014).

% \bibitem{Hennigar1} R. A. Hennigar, et al. \textit{J. High Energ. Phys.} \textbf{2020}, 27 (2020).
% \bibitem{Hennigar2} L. Ma and H. Lu, \textit{Eur. Phys. J. C} \textbf{80}, 1209 (2020).
% \bibitem{Hennigar3} A. casalino, et al. \textit{Phys. Dark Univ.} \textbf{31}, 100770 (2021).
% \bibitem{Eiesland} J. Eiesland, \textit{Trans. Am. Math. Soc.} \textbf{27}, 213 (1925).
% \bibitem{Eisenhart1} L. P. Eisenhart, \textit{Riemannian Geometry}, (Princeton University Press, Princeton, United States of America, 1966).
% \bibitem{Karmarkar1} K. R. Karmarkar, \textit{Proc. Indian Acad. Sci. A} \textbf{27} 56 (1948).
% \bibitem{Pandey1} S. N. Pandey and S. P. Sharma, \textit{Gen. Rel. Grav.} \textbf{14}, 113 (1981).
% \bibitem{Islam1} P. K. F. Kuhfittig, \textit{Eur. Phys. J. C} \textbf{ 74}, 2818 (2014).
% \bibitem{Islam3} F. Rahaman, P. Salucci, P. K. F. Kuhfittig, S. Ray, and M. Rahaman, \textit{Ann. Phys. }\textbf{350}, 561 (2014).
% \bibitem{Oort4} J. H.  Oort, \textit{Bull. Astro. Inst. Nether.} \textbf{3}, 275 (1927).
% \bibitem{Frenk2} J. F. Navarro, C. S. Frenk, and S. D. M. White, \textit{Astro. J.}, \textbf{462}, 563 (1996).
% \bibitem{Frenk3} J. F. Navarro, C. S. Frenk, and S. D. M. White, \textit{Astro. J.}, \textbf{490}, 493 (1997).
% \bibitem{Frenk44} D. Merritt et al., \textit{Astrophys. J.} \textbf{624}, L85 (2005).
% \bibitem{Frenk5} D. Merritt et al., \textit{Astrono. J.} \textbf{132}, 2685 (2006).
% \bibitem{Rizwan1} K. Jusufi, M. Jamil, and M. Rizwan, \textit{Gen. Rel. Grav.} \textbf{51}, 102 (2019).
% \bibitem{Rizwan2} Z. Xu, M. Tang, G. Cao, and S.-N. Zhang, \textit{Eur. Phys. J. C} \textbf{80}, 70 (2020).
% \bibitem{Rizwan4} G. Mustafa, S. K. Maurya, and S. Ray, \textit{Astrophys. J.} \textbf{941}, 170 (2022).
% % \bibitem{Burkertt} A. Burkert, \textit{Astro. J} \textbf{447}, L25-L28, (1995).
% % \bibitem{Stel} M. Persic, P. Salucci, F. Stel, \textit{MNRAS} \textbf{281}, 27 (1996).
% % \bibitem{Carlberg} J. Dubinski and R. G. Carlberg, \textit{Astro. J.} \textbf{378}, 496 (1991).
% \bibitem{Matos1} L. A. Urena-Lopez, T. Matos and R. Becerril, \textit{Class. Quant. Grav.} \textbf{19}, 6259 (2002).
% \bibitem{Matos2} T. Harko, \textit{J. Cosmo. Astro. Phys.} \textbf{05}, 022 (2011).
% % \bibitem{Hou1} X. Hou et al., \textit{J. Cosmo. Astro. Phys.} \textbf{2018}, 015 (2018).
% % \bibitem{Hou2} Z. Xu et al., \textit{J. Cosmo. Astro. Phys.} \textbf{2018}, 038(2018).
% \bibitem{Liempi1} M. Cataldo, L. Liempi, and P. Rodriguez, \textit{Phys. Lett. B} \textbf{757}, 130-135 (2016).
% \bibitem{Liempi2} F. S. N. Lobo, \textit{Phys. Rev. D} \textbf{71}, 084011 (2005).
% \bibitem{Liempi3} A. S. Nezhada, M. R. Mehdizadehb, and H. Golchin, \textit{Eur. Phys. J. Plus} \textbf{139}, 110 (2024).






% \bibitem{Sahdev} Kar and Sahdev, \textit{Phys. Rev. D} \textbf{52}, 2030 (1995).
% \bibitem{Anchordoqui} L. A. Anchordoqui et al., \textit{Phys. Rev. D} \textbf{57}, 829 (1998).
% \bibitem{Fayyaz1} M. F. Shamir and I. Fayyaz, \textit{Eur. Phys. J. C} \textbf{80}, 1102 (2020).
% \bibitem{Fayyaz2} A. Malik et al. \textit{Eur. Phys. J. C} \textbf{83}, 522 (2023).
% %\bibitem{Mustafa} G. Mustafa et al. \textit{Phys. Lett. B} \textbf{821}, 136612 (2021).
% \bibitem{Sarkar} S. Sarkar, N. Sarkar, and F. Rahaman \textit{Eur. Phys. J. C} \textbf{80}, 882 (2020).
% % \bibitem{Channuie11} K. Jusufi, P. Channuie, and M. Jamil, \textit{Eur. Phys. J. C} \textbf{80}, 127 (2020).
% % \bibitem{Hassan2} Z. Hassan, S. Ghosh, P. K. Sahoo, and V. S. Hari Rao, \textit{Gen. Relativ. Gravit.} \textbf{55}, 90 (2023).
% \bibitem{L. Herrera} L. Herrera, \textit{Phys. Rev. D} \textbf{97}, 044010 (2018).
% \bibitem{Gomez1} Alfonso Garcia-Parrado Gomez-Lobo, \textit{Class. Quantum Grav.} \textbf{25}, 015006 (2008).
% \bibitem{Gomez2} L. Herrera et al.,  \textit{Phys. Rev. D} \textbf{79}, 064025 (2009).
% \bibitem{Casadio1} R. Casadio et al., \textit{Eur. Phys. J. C} \textbf{79}, 826 (2019).
% \bibitem{Casadio2} E. Contreras and E. Fuenmayor, \textit{Phys. Rev. D} \textbf{103}, 124065 (2021).
% \bibitem{Casadio3} C. Arias, E. Contreras, E. Fuenmayor, and A. Ramos,\textit{ Ann. Phys.} \textbf{436}, 168671 (2022).
% %\bibitem{} R. Avalos, E. Fuenmayor, and E. Contreras, \textit{Eur. Phys. J. C} \textbf{82}, 420  (2022).
% \bibitem{Butt1} M. Sharif and I. I. Butt, \textit{Eur. Phys. J. C} \textbf{78}, 688 (2018).
% \bibitem{Butt2} Z. Yousaf, M. Yu. Khlopov, M. Z. Bhatti, and T. Naseer, \textit{MNRAS}  \textbf{495}, 4334-4346 (2020).
% \bibitem{Butt3} M. Zubair and M. Farooq, \textit{Eur. Phys. J. C} \textbf{83}, 507 (2023).
% \bibitem{Katz1} D. Lynden-Bell, J. Katz, J. Bicak, \textit{Phys. Rev. D} \textbf{75}, 024040 (2007).
% \bibitem{Katz2} K. K. Nandi, Y. Z. Zhang, R. G. Cai, and A. Panchenko, \textit{Phys. Rev. D} \textbf{79}, 024011 (2009).
% \bibitem{A. Wheeler} C. W. Misner, K. S. Thorne, and J. A. Wheeler, \textit{Gravitation} (Freeman, San Francisco, 1973), pp. 467 and 603.
% \bibitem{Manna1} P. Bhar, F. Rahaman, T. Manna, and A. Banerjee, \textit{Eur. Phys. J. C} \textbf{76}, 708 (2016).
% \bibitem{Manna2} F. Rahaman, S. Karmakar, I. Karar, and S. Ray, \textit{Phys. Lett. B} \textbf{746}, 73-78 (2015).
% \bibitem{Manna3} O. Sokoliuk, S. Mandal, P. K. Sahoo, and A. Baransky, \textit{Eur. Phys. J. C} \textbf{82}, 280 (2022).
% \bibitem{Rahaman7} F. Rahaman, P. K. F. Kuhfitting, S. Ray, and N. Islam, \textit{Eur. Phys. J. C} \textbf{74}, 2750 (2014).
% \bibitem{Atamurotov} G. Mustafa, F. Atamurotov, and Sushant G. Ghosh, \textit{Phys. Dark Univ.} \textbf{40}, 101214 (2023).
% \bibitem{Rizwan3} B. C. Paul, \textit{Class. Quant. Grav.} \textbf{38} 145022 (2021).
% %\bibitem{Sahoo} M. Tayde, Z. Hassan, and P. K. Sahoo, \textit{Nucl. Phys. B} \textbf{1000}, 116478 (2024).















































% % \bibitem{einstein} A. Einstein, Sitzungsber. Preuss. Akad. Wiss. Berlin (Math.Phys.) \textbf{1917}, 142 (1917).

% % \bibitem{desitter}W. de Sitter, Philosophical Problems in Science \textbf{63}, 205 (2017).

% % \bibitem{desitter2}W. de Sitter, MNRAS, \textbf{78}, 3 (1917).

% % \bibitem{friedman}A. Friedman, Zeitschrift für Physik \textbf{10}, 377 (1922).

% % \bibitem{lemaitre} G. Lemaitre, MNRAS \textbf{91}, 483 (1931).

% % \bibitem{penzias} A. A. Penzias, R. W. Wilson, Astrophys. J. \textbf{142}, 419 (1965).

% % \bibitem{riess/1998}A. G. Riess et al., Astron. J. \textbf{116}, 1009 (1998).
 
% % \bibitem{perlmutter/1999} S. Perlmutter et al., ApJ. \textbf{517}, 565 (1999).

% % \bibitem{planck/2015}P. A. R. Ade et al., Astron. Astrophys. \textbf{594}, A13 (2015).

% % \bibitem{dub} B. A. Dubrovin, A. T. Fomenko, S. P. Novikov, \textit{Modern Geometry-Methods and Applications: Part I: The Geometry of Surfaces, Transformation Groups, and Fields}, 2nd edition, (New York: Springer Verlag).

% % \bibitem{lan} L. D. Landau, E. M. Lifshitz, The Classical Theory of Fields, (Amsterdam: Butterworth-Heinemann, 1994).

% % \bibitem{hehl/1976} W. Hehl, et al., Rev. Mod. Phys. \textbf{48}, 393 (1976).

% % \bibitem{maluf}J. W. Maluf, 
% % %“The teleparallel equivalent of general relativity”, 
% % Annalen Phys. \textbf{525}, 339 (2013).

% % \bibitem{Haghani} Z. Haghani et al.,
% % %“Weyl-Cartan-Weitzenboeck gravity as a generalization of teleparallel gravity,” 
% % JCAP \textbf{1210}, 061 (2012).

% % \bibitem{nester}J. M. Nester, H. J. Yo,
% % % “Symmetric teleparallel general relativity,”
% %   Chin. J. Phys. \textbf{37}, 113 (1999).
  
% % \bibitem{olmo} G. J. Olmo, Int. J. Mod. Phys. D \textbf{20}, 413 (2011).

% % \bibitem{heisenberg} L. Heisenberg, Phys. Rep. \textbf{796}, 1 (2019).

% % \bibitem{heisenberg1} J. Beltr\'an Jim\'enez, L. Heisenberg, T. S. Koivisto, Universe \textbf{5}, 173 (2019).

% % \bibitem{r/1923} R. Weitzenb$\ddot{o}$ck, \textit{Invariantentheorie}, Noordhoff, Gronningen (1923).
% % \bibitem{Hayashi/1979} K. Hayashi, T. Shirafuji, Phys. Rev. D \textbf{19}, 3524 (1979).
% % \bibitem{Arcos/2004} H. I. Arcos, J. G. Pereira, Int. J. Mod. Phys. D \textbf{13}, 2193 (2004).
% % \bibitem{Maluf/1994} J. W. Maluf, J. Math. Phys. \textbf{35}, 335 (1994).


% % \bibitem{robert}H. P. Robertson, Astrophys. J. \textbf{82}, 284 (1935).

% % \bibitem{walker} A. G. Walker, Proc. Lon. Math. Soc. \textbf{42}, 90127 (1937).

% % \bibitem{1}W. Hillebrandt, J. C. Niemeyer, Ann. Rev. Astron. Astrophys. \textbf{38}, 191 (2000).

% % \bibitem{2} B. Leibundgut et al., ApJ. \textbf{466}, L21  (1996). 

% % \bibitem{3} S. Perlmutter et al., ApJ. \textbf{483}, 565 (1997).

% % \bibitem{4} B. Leibundgut, Ann. Rev. Astron. Astrophys. \textbf{39}, 67 (2001). 

% % \bibitem{7}J. Frieman, M. Turner, D. Huterer, Ann. Rev. Astron. Astrophys. \textbf{46}, 385 (2008).

% % \bibitem{9} J. L. Tonry et al., ApJ. \textbf{594}, 1 (2003).

% % \bibitem{10} B. Barris et al., ApJ. \textbf{602}, 571 (2004).

% % \bibitem{19}J. A. Holtzman et al., AJ. \textbf{136}, 2306 (2008); R. Kessler et al., ApJS. \textbf{185},  32 (2009).

% % \bibitem{18}J. Leaman et al., arXiv:1006.4611; W. D. Li et al., arXiv:1006.4612; W. D. Li et al., arXiv:1006.4613.

% % \bibitem{17} G. Folatelli et al., AJ. \textbf{139}, 120 (2010); G. Folatelli et al., AJ. \textbf{139} , 519 (2010).

% % \bibitem{16} Y. Copin et al., New Astronomy Rev. \textbf{50}, 436 (2006); R. A. Scalzo et al., ApJ. \textbf{713}, 1073 (2009).

% % \bibitem{15}G. Miknaitis et al., ApJ. \textbf{666}, 674 (2007); W. M. Wood-Vasey et al., ApJ. \textbf{666}, 694 (2007).

% % \bibitem{1314}P. Astier et al., Astron. Astrophys. \textbf{447}, 31 (2006);S. Baumont et al., Astron. Astrophys. \textbf{491}, 567 (2008); N. Regnault et al., arXiv:0908.3808; J. Guy et al., arXiv:1010.4743.

% % \bibitem{1112} A. G. Riess et al., ApJ. \textbf{607} 665 (2004); A. G. Riess et al., ApJ. \textbf{659}, 98 (2007). 

% % \bibitem{37} A. A. Penzias, R. W. Wilson, ApJ. \textbf{142} 419 (1965).

% % \bibitem{38} R. A. Alpher, H. Bethe, G. Gamow, Phys. Rev. D \textbf{73}, 803 (1948). 

% % \bibitem{39}G. F. Smoot et al., ApJ. \textbf{396}, Ll  (1992); C. L. Bennett et al., ApJ. \textbf{396},  L7 (1992). 

% % \bibitem{40} A. D. Miller et al., ApJL. \textbf{524}, L1 (1999); P. de Bernardlis et al., Nature

% % (London) \textbf{404}, 955 (2000); S. Hanany et al., ApJL. \textbf{545} L5 (2000).

% % \bibitem{41} P. J. E. Peebles, J. T. Yu, ApJ. \textbf{162}, 815 (1970).

% % \bibitem{42} J. R. Bond, G. Efstathiou, ApJ. \textbf{285} L45 (1984).

% % \bibitem{WAMP} D. N. Spergel et al., ApJS \textbf{148}, 175 (2003); H. V. Peiris et al., ApJS \textbf{148}, 213 (2003); D. N. Spergel et al., ApJS \textbf{170}, 377 (2007); E. Komatsu et al., ApJS \textbf{180}, 330 (2009).

% % \bibitem{Planck/2011} Planck Collaboration: arXiv: 1101.2022, arXiv: 1101.2023, arXiv: 1101.2024.

% % \bibitem{62} J. Silk, ApJ \textbf{151}, 459 (1968).

% % \bibitem{69} A. Albrecht et al., arXiv:astro-ph/0609591; J. Guzik, G. Bernstein, R. E. Smith, MNRAS \textbf{375}, 1329 (2007); H. J. Seo, D. J. Eisenstein, ApJ. \textbf{665} 14 (2007); R. E. Smith, R. Scoccimarro, R. K. Sheth, Phys. Rev. D \textbf{77}, 043525 (2008). 

% % \bibitem{72} M. Colless et al., arXiv:astro-ph/0306581.

% % \bibitem{73} D. G. York et al., AJ. \textbf{120}, 1579 (2000);  M. Tegmark et al., Phys. Rev. D \textbf{74}, 123507 (2006).

% % \bibitem{75} http://www.sdss3.org/dr8/.

% % \bibitem{136} E. Hubble, M. L. Humason, ApJ. \textbf{74}, 43  (1931).

% % \bibitem{138}W. L. Freedman et al., ApJ. \textbf{533}, 47 (2001).

% % \bibitem{139} A. Sandage et al., ApJ. \textbf{653}, 843 (2006).

% % \bibitem{140} A. G. Riess et al., ApJ. \textbf{699}, 539 (2009).

% % \bibitem{141}A. G. Riess et al., ApJ. \textbf{730}, 119 (2011).

% % \bibitem{145} W. L. Freedman, B. F. Madore, Annu. Rev. Astro. Astrophys. \textbf{48}, 673 (2010).

% % \bibitem{perkin} Miao Li, Xiao-Dong Li, Shuang Wang, Yi Wang, \textit{Dark Energy}
% % (Peking University Press-World Scientific Advanced Physics Series, 2014).

% % \bibitem{carroll/1992}S. M. Carroll et al., Annu. Rev. Astron. Astrophys. \textbf{30}, 499 (1992).
% % \bibitem{Sahni/2000} V. Sahni, A. Starobinski, Int. J. Mod. Phys. D, \textbf{9}, 373 (2000).

% % \bibitem{joyce/2016} A. Joyce et al., Ann. Rev. Nucl. Part. Sci., \textbf{66}, 95 (2016).

% % \bibitem{baker/2019} T. Baker et al., Rev. Mod. Phys. \textbf{93}, 15003 (2021).

% % \bibitem{peracaula/2019}J. S. Peracaula et al., Astrophys. J., \textbf{886}, L6 (2019); Y. Yerramsetti, et al., Eur. Phys. J. C, \textbf{79}, 1020 (2020); D. Wang, Phys. Dark Universe, \textbf{28}, 100545 (2020); D. Wang et al., Eur. Phys. J. C, \textbf{79}, 211 (2019); S. Arora et al., Class. Quan. Grav., 37, 205022 (2020); S. Bhattacharjee, P. K. Sahoo, Phys. Dark Universe, \textbf{28}, 100537 (2010).



% % \bibitem{bud} H. A. Buchdahl, Mon. Not. Roy. Astro. Soc. \textbf{150}, 1 (1970).

% % \bibitem{fr} A. A. Starobinsky, Physics Letters B \textbf{91}, 99 ( 1980); S .G. Chaudhury et al., Mon. Not. Roy. Astro. Soc., \textbf{485}, 5693 ( 2019); S. D. Odintsov, V. K Oikonomou, Phys. Rev. D  \textbf{101}, 044009 (2020);  A. G. Suvorov, Phys. Rev. D \textbf{99}, 124026 (2019); M. Zhang,R. B. Mann, Physi. Rev. D \textbf{100}, 084061 (2019); A. V. Astashenok, S. D. Odintsov, Mon. Not. Roy. Astro. Soc.  \textbf{493}, 78 (2020); P. Feola et al. Physi. Rev.D \textbf{101}, 044037 (2020).

% % \bibitem{Harko/2011}T Harko  et al., Phys. Rev. D \textbf{84}, 024020 (2011).

% % \bibitem{fg} D. Lovelock, J. Math. Phys., \textbf{12}, 498 (1971).

% % \bibitem{frlm} T. Harko, F. S. N. Lobo, Eur. Phys. J. C \textbf{70}, 373 (2010). 

% % \bibitem{ft} R. Ferraro,  F. Fiorini, Phys. Rev. D \textbf{75}, 084031 (2007).

% % \bibitem{ftb}S. Bahamonde, C. G. Böhmer, , M. Wright, Phys. Rev. D \textbf{92}, 104042 (2015).

% % \bibitem{ftg}G. Kofinas , E. N. Saridakis, Phys. Rev. D \textbf{90}, 084044 (2014).

% % %Chapter 2

% % %\bibitem{observations} A. G. Riess et al., Astron. J. \textbf{116}, 1009
% % %(1998); S. Perlmutter et al., Astrophys. J. \textbf{517}, 565 (1999); P.
% % %deBernardis et al., Nature \textbf{404}, 955 (2000); S. Perlmutter et al.,
% % %Astrophys. J. \textbf{598}, 102 (2003); M. Colless et al., Mon. Not. R.
% % %Astron. Soc. \textbf{328}, 1039 (2001); M. Tegmark et al., Phys. Rev. D 
% % %\textbf{69}, 103501 (2004); S. Cole et al., MNRAS 
% % %\textbf{362}, 505 (2005); V.Springel et al., Nature (London) \textbf{440},
% % %1137 (2006); P. A. R. Ade et al., Astron. Astrophys. \textbf{571}, A16
% % %(2014); P. Astier et al., Astron. Astrophys. \textbf{447}, 31 (2006); A. G.
% % %Riess et al., Astrophys. J. \textbf{659}, 98 (2007); D. N. Spergel et al.,
% % %Astrophys. J. Suppl. Ser. \textbf{148}, 175 (2003); H. V. Peiris et al.,
% % %Astrophys. J. Suppl. Ser. \textbf{148}, 213 (2003); D. N. Spergel et al.,
% % %Astrophys. J. Suppl. Ser. \textbf{170}, 377 (2007); E. Komatsu et al.,
% % %arXiv:0803.0547.
% % %
% % %\bibitem{alternate} B. Ratra, P. J. E Peebles, Phys. Rev. D \textbf{37},
% % %3406 (1988); R. R. Caldwell et al., Phys. Rev. Lett. \textbf{80}, 1582 1988;
% % %C. Armendariz-Picon et al., Phys. Rev. D \textbf{63}, 103510 (2001); T.
% % %Buchert, Gen. Relativ. Gravit. \textbf{32}, 105 (2000); P. Hunt, S. Sarkar,
% % %MNRAS \textbf{401}, 547 (2010); K. Tomita, Mon. Not. R.
% % %Astron. Soc. \textbf{326}, 287 (2001); B. Pandey, MNRAS 
% % %\textbf{485}, L73 (2019); B. Pandey, MNRAS \textbf{471},
% % %L77 (2017); K. A. Milton, Gravit. Cosmol.\textbf{\ 9}, 66 (2003); D. Easson
% % %et al., Phys. Lett. B \textbf{696}, 273 (2011); D. Pav\'on , N. Radicella,
% % %Gen. Relativ. Gravit. \textbf{45}, 63 (2013); N. Radicella, D. Pav\'on, Gen.
% % %Relativ. Gravit. \textbf{44}, 685 (2012).
% % %

% % %
% % %\bibitem{review} S. Nojiri et al., Phys. Rept. \textbf{692}, 1 (2017).
% % %\bibitem{snehasish}  P.K. Sahoo and S. Bhattacharjee, New Astronomy, \textbf{77}, 101351 (2020); R. Zaregonbadi, et al., Phys. Rev. D \textbf{94}, 084052 (2016); G. Sun and Y.-C. Huang, Int. J. Mod. Phys. D, \textbf{25}, 1650038 (2016); F. Rocha et al. arXiv:1911.08894 (2019); S.I. dos Santos, G.A. Carvalho, P.H.R.S. Moraes, C.H. Lenzi and M. Malheiro, Eur. Phys. J. Plus, \textbf{134}, 398 (2019); P.H.R.S. Moraes, J.D.V. Arban˜il and M. Malheiro, J. Cosm. Astrop. Phys. \textbf{06}, 005 (2016); P.H.R.S. Moraes and P.K. Sahoo, Eur. Phys. J. C \textbf{79}, 677 (2019); E. Elizalde and M. Khurshudyan, Phys. Rev. D, \textbf{99}, 024051 (2019); P.H.R.S. Moraes, W. de Paula and R.A.C. Correa, Int. J. Mod. Phys. D, \textbf{28}, 1950098 (2019); E. Elizalde and M. Khurshudyan, Phys. Rev. D, \textbf{98}, 123525 (2018); P.H.R.S. Moraes and P.K. Sahoo, Phys. Rev. D, \textbf{97}, 024007 (2018); P.K. Sahoo, P.H.R.S. Moraes and P. Sahoo, Eur. Phys. J. C, \textbf{78}, 46 (2018); P.K. Sahoo, P.H.R.S. Moraes, P. Sahoo and G. Ribeiro, Int. J. Mod. Phys. D, \textbf{27}, 1950004 (2018); P.H.R.S. Moraes and P.K. Sahoo, Phys. Rev. D, \textbf{96}, 044038 (2017); P.H.R.S. Moraes, R.A.C. Correa and R.V. Lobato, J. Cosm. Astrop. Phys., \textbf{07}, 029 (2017); T. Azizi, Int. J. Theor. Phys. \textbf{52}, 3486 (2013); M. Sharif and A. Siddiqa, Gen. Rel. Grav., \textbf{51}, 74 (2019);  M.E.S. Alves, P.H.R.S. Moraes, J.C.N. de Araujo and M. Malheiro, Phys. Rev. D, \textbf{94}, 024032 (2016); P.K. Sahoo and S. Bhattacharjee, Int. J. Theor. Phys, DOI: 10.1007/s10773-020-04414-3 [arXiv: 1907.13460]; S. Bhattacharjee and P. K. Sahoo, Eur. Phys. J. C. \textbf{80}, 289 (2020) [arXiv: 2002.11483]; 
% % % P. Sahoo et al, Mod. Phys. Lett. A, DOI: 10.1142/S0217732320500959 [arXiv: 1907.08682] ;S. Bhattacharjee and P. K. Sahoo, Phys. Dark. universe. \textbf{28}, 100537 (2020) [arXiv: 2003.14211]; S. Bhattacharjee and P. K. Sahoo, Eur. Phys. J. Plus, \textbf{135}, 86 (2020) [arXiv:2001.06569]; S. Bhattacharjee and P. K. Sahoo, Eur. Phys. J. Plus, DOI: 10.1140/epjp/s13360-020-00361-4.
% % \bibitem{cosmo7to9} G. R. Bengochea, R. Ferraro, Phys. Rev. D \textbf{79},
% % 124019 (2009); R. Ferraro, F. Fiorini, Phys. Rev. D \textbf{75}, 084031
% % (2007); E. V. Linder, Phys. Rev. D \textbf{81}, 127301 (2010).

% % \bibitem{reviewft} Y. F. Cai et al., Rept. Prog. Phys. \textbf{79},
% % 106901 (2016).

% % \bibitem{cosmoft} A. Paliathanasis et al., Phys. Rev. D \textbf{94}, 023525 (2016).

% % \bibitem{cosmo10to12} K. Hayashi, T. Shirafuji, Phys. Rev. D \textbf{19},
% % 3524 (1979); M. Tsamparlis, Phys. Lett. A \textbf{75}, 27 (1979); H. I.
% % Arcos, J.G. Pereira, Int. J. Mod. Phys. D \textbf{13}, 2193 (2004).

% % \bibitem{cosmo14} A. Einstein 1928, Sitz. Preuss. Akad. Wiss. p. 217; ibid
% % p. 224 [Translated by A. Unzicker, T. Case, (preprint: arXiv:
% % physics/0503046)]

% % \bibitem{cosmo19to20} K. Atazadeh, F. Darabi, Eur. Phys. J. C \textbf{72},
% % 2016 (2012); S. Basilakos et al., Phys. Rev. D \textbf{88}, 103526 (2013).

% % \bibitem{cosmo21} M. E. Rodrigues et al., Astroph. Space Sci. \textbf{357},
% % 129 (2015)

% % \bibitem{cosmo22to23} A. Paliathanasis et al., Phys. Rev. D \textbf{89},
% % 104042 (2014); S. Capozziello et al., JHEP \textbf{89}, 039 (2013).


% % \bibitem{inflation} K. Bamba et al., Phys. Rev. D \textbf{94}, 083513 (2016).

% % \bibitem{late} G. R. Bengochea, R. Ferraro, Phys. Rev. D \textbf{79}, 124019
% % (2009); K. Bamba et al., JCAP \textbf{01}, 021 (2011); R. Myrzakulov, Eur.
% % Phys. J. C \textbf{71}, 1752 (2011).

% % \bibitem{bounce} Y.F. Cai et al., Class. Quant. Grav. \textbf{28}, 215011
% % (2011); J. de Haro, J. Amor\'os, J. Phys. Conf. Ser. \textbf{600}, 012024
% % (2015); W. El Hanafy, G.
% % G. L. Nashed, Int. J. Mod. Phys. D \textbf{26}, 1750154 (2017).

% % \bibitem{bhatti/2017} M. Zaeem-ul-Haq Bhatti, Z.Yousaf, Sonia Hanif, Phys.
% % Dark Univ.,\textbf{16}, 34 (2017).

% % \bibitem{bhatti/2017a} M. Zaeem-ul-Haq Bhatti, Z.Yousaf, Sonia Hanif, Mod.
% % Phys. Lett. A, \textbf{32}, 1750042 (2017).

% % \bibitem{pacif} S. K. J. Pacif et al., Int. J. Geom. Meth. Mod. Phys. 
% % \textbf{14}, 1750111 (2017).

% % \bibitem{para} M. Chevallier, D. Polarski, Int. J. Mod. Phys. D \textbf{10},
% % 213 (2001); Mod. Phys. Lett. A. \textbf{35}, 2050011 (2020); S. del Campo et
% % al., Phys. Rev. D \textbf{86}, 083509 (2012); A. A. Mamon, K.Bamba, Eur.
% % Phys. J. C \textbf{78}, 862 (2018).

% % \bibitem{banerjee} N. Banerjee, S. Das, Gen. Relativ. Gravit. \textbf{37},
% % 1695 (2005).

% % \bibitem{olive21} S. Pan, A.Mukherjee, N.Banerjee, MNRAS 
% % \textbf{477}, 1189 (2018).

% % \bibitem{sahni} V. Sahni, T. D. Saini, A. A. Starobinsky, U. Alam: JETP
% % Lett. \textbf{77}, 201 (2003); U. Alam et al., MNRAS 
% % \textbf{344}, 1057 (2003).

% % \bibitem{sahni17to18} J. Albert et al. [SNAP Collaboration]: arXiv:0507458;
% % J. Albert et al. [SNAP Collaboration]: arXiv:0507459.

% % \bibitem{Omsahni} V. Sahni et al., Phys. Rev. D. \textbf{78}, 103502 (2008);
% % M. Shahalam1, Sasha Sami, Abhineet Agarwal, MNRAS 
% % \textbf{448} 2948 (2015); Abhineet Agarwal et al., Int. J. Mod. Phys. D %
% % \textbf{28} 1950083 (2019).

% % \bibitem{sahoo} P. H. R. S. Moraes, P. K. Sahoo, Eur. Phys. J. C. \textbf{77}%
% % , 480 (2017).

% % \bibitem{non39} R. M. Wald, General relativity (University of Chicago Press,
% % Chicago, 1984)

% % \bibitem{Poisson/2004} A. Raychaudhuri, Phys. Rev., \textbf{98} (1955) 1123; J.~Ehlers, Int. J. Mod. Phys. D,  \textbf{15}, 1573 (2006); S. Nojiri, S. D. Odintsov, Int. J. Geom. Methods Mod. Phys., \textbf{4}, 115 (2007).

% % \bibitem{energy} D. Liu, M. J. Reboucas, Phys.Rev. D. \textbf{86}, 083515
% % (2012); T. Azizi, M. Gorjizadeh, EPL \textbf{117}, 6 (2017);M. Zubair, Saira
% % Waheed, Astrophys Space Sci. \textbf{355}, 361 (2015).

% % \bibitem{sharov} G. S. Sharov, V. O. Vasiliev, Mathematical Modelling and
% % Geometry \textbf{6}, 1 (2018).

% % \bibitem{Hz1} C. H. Chuang, Y. Wang, MNRAS \textbf{435}%
% % , 255 (2013); C-H Chuang C-H. et al., MNRAS \textbf{433%
% % }, 3559 (2013); A. Font-Ribera et al., J. Cosmol. Astropart. Phys. \textbf{05%
% % }, 027 (2014); T. Delubac et al., Astron. Astrophys. \textbf{574}, id. A59,
% % 17 (2015); L.,erson et al., MNRAS \textbf{441}, 24
% % (2014); Y. Wang et al., MNRAS \textbf{469}, 3762
% % (2017); E. Gaztanaga et al. MNRAS \textbf{399}, 1663
% % (2009); C. Blake et al., MNRAS \textbf{425}, 405
% % (2012); N. G. Busca et al., Astro. Astrophys. \textbf{552}, A96 (2013); A.
% % Oka et al., MNRAS \textbf{439}, 2515 (2014); S. Alam
% % et al., MNRAS \textbf{470}, 2617 (2017); J. E.
% % Bautista et al., Astron. Astrophys. \textbf{603}, A12 (2017).

% % \bibitem{Hz2} J. Simon, L. Verde, R. Jimenez, Phys. Rev. D \textbf{71},
% % 123001 (2005); D. Stern et al., J. Cosmol. Astropart. Phys. \textbf{02}, 008
% % (2010); C. Zhang et al., Research in Astron. and Astrop. \textbf{14}, 1221
% % (2014); M. Moresco et al., J. Cosmol. Astropart. Phys. \textbf{8}, 006
% % (2012); M. Moresco, MNRAS: Letters., \textbf{450}, L16
% % (2015); M. Moresco M. et al., J. Cosmol. Astropart. Phys. \textbf{05}, 014
% % (2016); A. L. Ratsimbazafy et al., MNRAS \textbf{467},
% % 3239 (2017)

% % \bibitem{SNeIa} N. Suzuki et al., ApJ., \textbf{746}, 85 (2012).

% % \bibitem{padn} N. Padmanabhan, X. Xu, D. J. Eisenstein, R. Scalzo, A. J.
% % Cuesta, K. T. Mehta et al., MNRAS \textbf{427},
% % 2132 (2012).

% % \bibitem{6df} F. Beutler et al., MNRAS \textbf{416}, 3017 (2011).

% % \bibitem{boss} BOSS collaboration, L. Anderson et al., Mon. Not. Roy.
% % Astron. Soc. \textbf{441}, 24 (2014).

% % \bibitem{wig} C. Blake et al., MNRAS \textbf{425}, 405 (2012).

% % %\bibitem{adep} Ade P A R et al., Planck 2015 results. XIII. Cosmological
% % %parameters, Preprint arXiv:1502.01589 (2015)

% % \bibitem{waga} M. Vargas dos Santos, Ribamar R. R. Reis, J. Cosm. Astropart.
% % Phys., \textbf{1602}, 066 (2016).

% % \bibitem{gio} R. Giostri, M. V. d. Santos, I. Waga, R. R. R. Reis, M. O.
% % Calvao, B. L. Lago, JCAP \textbf{1203}, 027 (2012).

% % \bibitem{hing} G. Hinshaw et al., Astrophys. J. Suppl., \textbf{208},
% % 19 (2013).

% % \bibitem{non41to42} M. Visser, C. Barcelo. arXiv:gr-qc/0001099; C. Barcelo,
% % M. Visser, Int. J. Mod. Phys. D \textbf{11}, 1553 (2002).

% % \bibitem{Planck/2018} Planck Collaboration: arXiv:1807.06209.

% % \bibitem{Jaime/2019} B. S. Haridasu, V. V. Lukovic, M. Moresco, N. Vittorio,
% % J. Cosmol. Astropart. Phys. \textbf{10}, 015 (2018); J. R. Garza et al.,
% % Eur. Phys. J. C \textbf{79}, 890 (2019); Hai-Nan Lin, Xin Li, Li Tang, Chin.
% % Phys. C \textbf{43}, 075101 (2019); J. F. Jesus, R. Valentim, A. A. Escobal,
% % S. H. Pereira, arXiv: 1909.00090. 


% % %Chapter-3

% % %\bibitem{Capozziello_book} S. Capozziello, and V. Faraoni, \textit{Beyond Einstein Gravity: A Survey of Gravitational Theories for Cosmology and Astrophysics}, Springer Dordrecht, 2011. doi: 10.1007/978-94-007-0165-6.
% % %\bibitem{lv_papers} B. P. Abbott et al. (LIGO Scientific Collaboration and Virgo Collaboration), {\it Phys. Rev. Lett.}, {\bf 116} (2016) 061102; B. P. Abbott et al. (LIGO Scientific Collaboration and Virgo Collaboration),{\it Phys. Rev. Lett.},  {\bf 119} (2017) 161101; B. P. Abbott et al. (LIGO Scientific Collaboration and Virgo Collaboration), {\it Phys. Rev. Lett.},  {\bf 123} (2019) 011102.
% % %\bibitem{eht_papers} The Event Horizon Telescope Collaboration et al., {\it ApJL},  {\bf 875} (2019) L1; The Event Horizon Telescope Collaboration et al., {\it ApJL},  {\bf 875} (2019) L5. 

% % \bibitem{Lazkoz/2019} R. Lazkoz et al.,  Phys. Rev. D, {\bf 100}, 104027  (2019). 
% % \bibitem{Capozziello/2018} S. Capozziello et al., Phys. Lett. B, {\bf 781}, 99  (2018).

% % %\bibitem{Plank/2018} Planck Collaboration, arXiv:1807.06209.
% % \bibitem{Capozziello/2019} S. Capozziello et al., Int. J. Mod. Phys. D, \textbf{28}, 1930016 (2019). 
% % \bibitem{Riess/1998} A. G. Riess, et al., Astro. J., \textbf{116}, 1009 (1998); S. Perlmutter, et al., Astrophys. J., \textbf{517} 565 (1999); S. Perlmutter, et al., Astrophys. J., \textbf{598}  102 (2003); S. Cole, et al., Mon. N. Roy. Astro. Soc., \textbf{362}, 505 (2005); P. A. R. Ade, et al., Astron. Astrophys., \textbf{571}, A16 (2014). 
% % \bibitem{Santos/2007} J. Santos, et al., Phys. Rev. D, \textbf{76}, 083513  (2007).
% % \bibitem{Bertolami/2009} O. Bertolami, M. C. Sequeira, Phys. Rev. D, \textbf{79}, 104010 (2009).
% % \bibitem{Gracia/2011} N. M. Gracia et al., Phys. Rev. D, \textbf{83}, 104032  (2011).
% % \bibitem{Bamba/2017} K Bamba et al., Gen. Rel. Grav.,  \textbf{49}, 112 (2017).
% % \bibitem{Liu/2012} D. Liu, M. J. Rebouc,  Phys. Rev. D, \textbf{86}, 083515 (2012).
% % \bibitem{Sharif/2016} M. Sharif, A. Ikram, Eur. Phys. J. C, \textbf{76}, 640 (2016).
% % \bibitem{Sharif/2013} M. Sharif, M. Zubair, J. High Energy Physics, \textbf{2013}, 79 (2013).
% % \bibitem{Atazadeh/2014} K. Atazadeh, F. Darabi, Gen. Rel. Grav.,  \textbf{46}, 1664 (2014).
% % \bibitem{Yousaf/2018} Z. Yousaf et al. Int. J. Geom. Methods Mod. Phys.,  \textbf{15}, 1850146 (2018).
% % \bibitem{Moraes/2019} P.H.R.S. Moraes et al. Adv. Astron.,  \textbf{2019}, 8574798 (2019).
% % \bibitem{Harko/2018}T. Harko, et al., Phys. Rev. D, \textbf{98}, 084043 (2018). 
% % \bibitem{Visser/2000} M. Visser, C. Barcelo, COSMO-99, 98 (2000).
% % %\bibitem{Moraes/2017} P.H.R.S. Moraes, P.K. Sahoo, Eur. Phys. J. C, \textbf{77} 480 (2017).
% % \bibitem{Whinnett/2004} A. W. Whinnett, D. F. Torres, Astrophys. J., {\bf 603}, L133  (2004).
% % \bibitem{Calcagni_book} G. Calcagni, \textit{Classical and Quantum Cosmology}, Springer Switzerland, 2017.

% % %Chapter-4

% % %\bibitem{riess/1998} A. G. Riess, et al., \textit{Astron. J.} \textbf{116}, 1009 (1998);  S. Perlmutter, et al., \textit{Astrophys. J.} \textbf{517}, 565 (1999); S. Perlmutter, et al., \textit{Astrophys. J.} \textbf{598}, 102 (2003);  D. N. Spergel,  et al.,  \textit{Astrophys. J. Suppl. Ser.} \textbf{148}, 175 (2003); A. G. Riess, et al., \textit{Astrophys. J.} \textbf{659}, 98 (2007);  D. N. Spergel,  et al.,  \textit{Astrophys. J. Suppl. Ser.} \textbf{170}, 377 (2007).
% % %
% % %\bibitem{carroll/1992}S. M. Carroll et al., \textit{Annu. Rev. Astron. Astrophys.} \textbf{30}, 499 (1992); V. Sahni, A. Starobinski, \ijmpd, \textbf{9}, 373 (2000).
% % %
% % %\bibitem{yang/2010}R. J. Yang, S. N. Zhang, \mnras,  \textbf{407}, 1835 (2010).
% % %
% % %\bibitem{veltan/2014} H. E. S. Velten ey al., Eur. Phys. J. C, \textbf{74}, 3160 (2014).
% % %
% % %\bibitem{joyce/2016} A. Joyce et al., \textit{Ann. Rev. Nucl. Part. Sci.}, \textbf{66}, 95 (2016).
% % %
% % %\bibitem{baker/2019} T. Baker et al., (2019), arXiv:1908.03430.
% % %
% % %\bibitem{peracaula/2019}J. S. Peracaula et al., \textit{Astrophys. J.}, \textbf{886}, L6 (2019); S. Mandal et al., \textit{Phys. Dark Universe}, \textbf{28}, 100551 (2020); Y. Yerramsetti, et al., Eur. Phys. J. C, \textbf{79}, 1020 (2020); D. Wang, \textit{Phys. Dark Universe}, \textbf{28}, 100545 (2020); D. Wang et al., Eur. Phys. J. C, \textbf{79}, 211 (2019); S. Arora et al., \cqg, 37, 205022 (2020); S. Bhattacharjee and P. K. Sahoo, \textit{Phys. Dark Universe}, \textbf{28}, 100537 (2010).
% % %
% % %\bibitem{hehl/1995}F. W. Hehl et al., \textit{Phys. Rep.} \textbf{258}, 1 (1995); T. Ortin, \textit{Gravity and Strings} (Cambridge University Press, Cambridge, England, 2015).
% % %
% % %\bibitem{aldrovandi/2014}R. Aldrovandi and J. Pereira, \textit{Teleparallel Gravity. An Introduction}, Fundamental Theories of Physics Vol. 173 (Springer, Dordrecht, 2014).
% % %
% % %\bibitem{maluf/2013}J. W. Maluf, \textit{Ann. Phys.}, \textbf{525}, 339 (2013).
% % %
% % %\bibitem{haghani/2012} Z. Haghani et al., \jcap, \textbf{10}, 061 (2012).
% % %
% % %\bibitem{haghani/2013}Z. Haghani et al., Phys. Rev. D, \textbf{88}, 044024 (2013).
% % %
% % %\bibitem{nester/1999}J. M. Nester and H.-J. Yo, \textit{Chin. J. Phys.} \textbf{37}, 113 (1999).
% % %
% % %\bibitem{ferraro/2008}R. Ferraro and F. Fiorini, Phys. Rev. D, \textbf{78}, 124019 (2008); E. V. Linder, Phys. Rev. D, \textbf{81}, 127301 (2010); Y.-F. Cai et al., \textit{Rep. Prog. Phys.} \textbf{79}, 106901 (2016); C.-Q. Geng et al., \textit{Phys. Lett. B}, \textbf{704}, 384 (2011); L. Jarv and A. Toporensky, Phys. Rev. D, \textbf{93}, 024051 (2016); J. B. Jim´enez et al., Phys. Rev. D, \textbf{98}, 044048 (2018); A. Conroy and T. Koivisto, Eur. Phys. J. C, \textbf{78}, 923 (2018).
% % %
% % %\bibitem{jarv/2018} L. J\"arv et al., Phys. Rev. D, \textbf{97}, 124025 (2018).
% % %
% % %\bibitem{hehl/1976} F. W. Hehl, et al., \textit{Rev. Mod. Phys.}, \textbf{48}, 393 (1976).

% % %\bibitem{Lazkoz/2019}R. Lazkoz et al.,Phys. Rev. D, \textbf{100}, 104027 (2019).

% % \bibitem{Mandal/2020} S. Mandal, P.K. Sahoo, J.R.L. Santos, Phys. Rev. D, \textbf{102}, 024057  (2020).

% % \bibitem{jianbo/2019} J. Lu et al., Eur. Phys. J. C, \textbf{79}, 530 (2019).

% % \bibitem{mikhel/2018} M. R\"unkla, O. Vilson, Phys. Rev. D, 98, 084034 (2018).

% % \bibitem{viktor/2020}V. Gakis, et al., Phys. Rev. D, \textbf{101}, 064024 (2020).

% % %\bibitem{Harko/2018} T. Harko, et al., Phys. Rev. D, \textbf{98}, 084043 (2018).

% % \bibitem{olmo/2015} G. J. Olmo, D. Rubiera-Garcia, Phys. Lett. B, \textbf{740}, 73 (2015).

% % \bibitem{einstein/1916}A. Einstein, Hamiltonsches Prinzip und allgemeine Relativit\"atstheorie, K\"oniglich Preu$\mathcal{B}$ische, Akademie der Wissenschaften (Berlin), Sitzungsberichte (1916), pp. 1111-1116.



% % %\bibitem{Jimenez/2018} J. B. Jim\'enez, L. Heisenberg, T. Koivisto, Phys. Rev. D, 
% % %\textbf{98}, 044048 (2018).

% % \bibitem{tomi/2018} T. Koivisto, Int. J. Geom. Methods Mod. Phys., \textbf{15}, 1840006 (2018).

% % \bibitem{Cattoen/2008}C. Cattoen, M. Visser, Phys. Rev. D, \textbf{78}, 063501 (2008); A. Aviles, et al., Phys. Rev. D, \textbf{87}, 044012 (2013); A. Aviles, et al., Phys. Rev. D, \textbf{86}, 123516 (2012); S. Capozziello, et al., Phys. Rev. D, \textbf{78}, 063504 (2008). 

% % \bibitem{will/2006}C. M. Will, Living Rev. Relativity, \textbf{9}, 3 (2006).


% % \bibitem{Scolnic/2018} D.~M.~Scolnic {\it et al.}, Astrophys.\ J.\  {\bf 859}, 101 (2018).

% % \bibitem{hobson/2009} M. P. Hobson, A. H. Jaffe, A. R. Liddle, P. Mukherjee, D.Parkison, \textit{Bayesian Methods in Cosmology}, (Cambridge University Press, Cambridge, 2009).

% % %Chapter-5







% % %\bibitem{Harko_2011} T. Harko et al., \textit{Phys. Rev. D}, {\bf 84}  (2011) 024020.

% % \bibitem{Ray_1955} A. Raychaudhuri, Phys. Rev., {\bf 98}, 1123 (1955).


% % \bibitem{Carroll_2004} S. Carroll, Spacetime and Geometry, An Introduction to GR (Addison Wesley, Boston 2004).

% % \bibitem{Hawking_1973} S.W. Hawking, G. F. R Ellis, The Large Scale Structure of Spacetime (Cambridge Univ Press, Cambridge 1973).

% % \bibitem{Bamba_2017} K. Bamba et al., Gen. Relativ. Gravit., {\bf 49}, 112 (2017).

% % \bibitem{Capo_2018} S. Capozziello et al., Phys. Lett. B, {\bf 781}, 99 (2018).

% % \bibitem{Atazadeh_2014} K. Atazadeh, F. Darabi, Gen. Relativ. Gravit., {\bf 46}, 1664 (2014).

% % \bibitem{Zubair_2015} M. Zubair, S. Waheed, Astrophys. Space. Sci., {\bf 355}, 361 (2015).

% % %\bibitem{Planck} Planck Collaboration, arXiv:1807.06209.

% % %\bibitem{Poisson/2004}  J.~Ehlers, Int. J. Modern Phys. D,  \textbf{15} (2006) 1573; S. Nojiri, S. D. Odintsov, \textit{Int. J. Geom. Methods Mod. Phys.}, \textbf{4} (2007) 115.

% % %\bibitem{Capozziello/2019} S. Capozziello et al., Int. J. Modern Phys. D, \textbf{28} (2019) 1930016.





% % %Chapter-6
% % %\bibitem{Capo/2011} S. Capozziello, M. De Laurentis, \href{https://www.sciencedirect.com/science/article/pii/S0370157311002432}{Phys. Rep. \textbf{509}, 167 (2011)}.
% % %
% % %\bibitem{Sari} E. N. Saridakis, et al., CANTATA, \href{https://arxiv.org/abs/2105.12582}{arXiv:2015.12582}.

% % %\bibitem{Jimenez/2018} J. B. Jimenez, L. Heisenberg, and T. Koivisto, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.98.044048}{Phys. Rev. D \,\ \textbf{98}, 044048 (2018)}.

% % %\bibitem{Lazkoz/2019} R. Lazkoz et al,, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.100.104027}{Phys. Rev. D \,\ \textbf{100}, 104027 (2019)}.

% % %\bibitem{Mandal/2020} S. Mandal, P.K. Sahoo, J.R.L. Santos, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.102.024057}{Phys. Rev. D \,\ \textbf{102}, 024057 (2020)}.

% % \bibitem{Mandal/2020a}S. Mandal, D. Wang, P.K. Sahoo, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.102.124029}{Phys. Rev. D \,\ \textbf{102}, 124029 (2020)}.

% % %\bibitem{Harko/2018}T. Harko et al,, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.98.084043}{Phys. Rev. D \,\ \textbf{98}, 084043 (2018)}.

% % \bibitem{Barros/2020} B. J. Barros et al., \href{https://www.sciencedirect.com/science/article/pii/S2212686420302387?via\%3Dihub}{Phys. Dark Universe \textbf{30}, 100616 (2020)}.
 
% % \bibitem{Jimenez/2020} J. B. Jimenez et al,, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.101.103507}{Phys. Rev. D \,\ \textbf{101}, 103507 (2020)}.

% % \bibitem{Hasan/2021}Z. Hasan, S. Mandal, P.K. Sahoo, \href{https://onlinelibrary.wiley.com/doi/10.1002/prop.202100023}{Fortschritte der Physik \textbf{69}, 2100023 (2021)}.

% % \bibitem{Solanki/2021}R. Solanki et al., \href{https://www.sciencedirect.com/science/article/pii/S2212686421000510?via\%3Dihub}{Phys. Dark Universe \textbf{32}, 100820 (2021)}.

% % \bibitem{Frus/2021} N. Frusciante, \href{https://www.scopus.com/record/display.uri?eid=2-s2.0-85101007939&origin=inward}{Phys. Rev. D \,\ \textbf{103}, 044021 (2021)}.

% % \bibitem{Flat/2021} K. Flathmann, M. Hohmann, \href{https://www.scopus.com/record/display.uri?eid=2-s2.0-85100981932&origin=inward}{Phys. Rev. D \,\ \textbf{103}, 044030 (2021)}.

% % \bibitem{Khyllep/2021} W. Khyllep, A. Paliathanasis, J. Dutta, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.103.103521}{Phys. Rev. D \,\ \textbf{103}, 103521 (2021)}.

% % \bibitem{Anag/2021} F. K. Anagnostopoulos, S. Basilakos, E. N. Saridakis, \href{https://www.sciencedirect.com/science/article/pii/S0370269321005748?via\%3Dihub}{Phys. Lett. B \,\ \textbf{822}, 136634 (2021)}.

% % \bibitem{Ata/2021} L. Atayde, N. Frusciante, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.104.064052}{Phys. Rev. D \,\ \textbf{104}, 064052 (2021)}.

% % \bibitem{Dial/2019}K. F. Dialektopoulos, T. S. Koivisto, S. Capozziello, \href{https://link.springer.com/article/10.1140/epjc/s10052-019-7106-8}{Eur. Phys. J. C \,\ \textbf{79}, 606 (2019)}. 

% % \bibitem{Ayu/2021}I. Ayuso, R. Lazkoz, V. Salzano, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.103.063505}{Phys. Rev. D \,\ \textbf{103}, 063505 (2021)}.

% % \bibitem{Amb/2020}F. D'Ambrosio, M. Garg, L. Heisenberg, \href{https://www.sciencedirect.com/science/article/pii/S0370269320307735}{Phys. Lett. B \,\ \textbf{811}, 135970 (2020)}.

% %\bibitem{baye}\href{http://www.cambridge.org/us/catalogue/catalogue.asp?isbn=9780521887946}{Bayesian Methods in Cosmology, edited by M. P. Hobson, A. H. Jaffe, A. R. Liddle, P. Mukherjee, and D. Parkison (Cambridge University Press, Cambridge, England, 2009)}.

% %\bibitem{Sharov/2018} G. S. Sharov, V. O. Vasiliev, \href{https://mmg.tversu.ru/images/publications/2018-611-abstract-references.pdf}{Mathematical Modelling and Geometry, \textbf{6}, 1 (2018)}.
% %
% %\bibitem{BAO1} C. H. Chuang, Y. Wang,\href{https://doi.org/10.1093/mnras/stt1290}{MNRAS \,\ \textbf{435}, 255 (2013)}.
% %
% %\bibitem{BAO2} C-H Chuang C-H. et al., \href{https://doi.org/10.1093/mnras/stt988}{MNRAS \,\ \textbf{ 433}, 3559  (2013)};  
% % 
% % \bibitem{BAO3} T.  Delubac  et  al.,  \href{https://www.aanda.org/articles/aa/full_html/2015/02/aa23969-14/aa23969-14.html}{Astron. Astrophys. \,\ \textbf{574}, 17 (2015)}; 
% %  
% % \bibitem{BAO4}L. Anderson et al., \href{https://doi.org/10.1093/mnras/stu523}{MNRAS \,\ \textbf{441}, 24 (2014)}; 
% % 
% %  
% % \bibitem{BAO5}S. Alam et al., \href{https://doi.org/10.1093/mnras/stx721}{MNRAS \,\ \textbf{470}, 2617 (2017)}. 
% % 
% % \bibitem{h1} J. Simon, L. Verde, R. Jimenez, \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.71.123001}{ Phys. Rev. D \,\ \textbf{71}, 123001 (2005)}.
% % 
% % \bibitem{h2}D. Stern et al., \href{https://iopscience.iop.org/article/10.1088/1475-7516/2010/02/008/meta}{JCAP \,\ \textbf{02}, 008 (2010)}.
% %  
% %\bibitem{h3}M. Moresco, \href{https://doi.org/10.1093/mnrasl/slv037}{MNRAS \,\ \textbf{450},  L16 (2015)}.
% %
% %\bibitem{h4} A. L. Ratsimbazafy et al., \href{https://doi.org/10.1093/mnras/stx301}{MNRAS \,\ \textbf{467}, 3239 (2017)}.

% %\bibitem{Scolnic/2018}D. M. Scolnic et al., \href{https://iopscience.iop.org/article/10.3847/1538-4357/aab9bb}{Astrophys. J. \,\ \textbf{859}, 101 (2018)}.

% %\bibitem{capo/2014} S. Capozziello et al., \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.90.044016}{Phys. Rev. D \,\ \textbf{90}, 044016 (2014)}.

% %\bibitem{capo/2019} S. Capozziello, R. D'Agostino, Orlando Luongo, \href{https://www.worldscientific.com/doi/abs/10.1142/S0218271819300167}{Int. J. Modern Phys. D \,\ \textbf{28}, 1930016 (2019).}

% %\bibitem{capo/2011} S. Capozziello et al., \href{https://journals.aps.org/prd/abstract/10.1103/PhysRevD.84.043527}{Phys. Rev. D \,\ \textbf{84}, 043527 (2011)}.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








\end{thebibliography}

==> variables2.tex <==
%-------------------------------------------------------------------------------
%	DOCUMENT VARIABLES
%
%	Fill in the lines below to set the various variables for the document
%-------------------------------------------------------------------------------

%-------------------------------------------------------------------------------
% Your thesis title - this is used in the title and abstract
% Command: \ttitle
\thesistitle{Astrophysical Objects in Modified Theories
of Gravity}
%-------------------------------------------------------------------------------
% The document type: Thesis / report, etc.
% Command: \doctype
\documenttype{\textbf{SYNOPSIS}}
%-------------------------------------------------------------------------------
% Your supervisor's name - this is used in the title page
% Command: \supname
\supervisor{\textbf{Prof. Pradyumn Kumar Sahoo}}
%-------------------------------------------------------------------------------
% The supervisor's position - Used on Certificate
% Command: \suppos
\supervisorposition{\textbf{Professor}}
%-------------------------------------------------------------------------------
% Supervisor's institute
% Command: \supinst
\supervisorinstitute{\textbf{BITS, Pilani, Hyderabad Campus}}
%-------------------------------------------------------------------------------
% Your Co-Supervisor's name
% Command: \cosupname
%\cosupervisor{Dr. Pradyumn Kumar Sahoo}
%-------------------------------------------------------------------------------
% Co-Supervisor's Position - Used on Certificate
% Command: \cosuppos
%\cosupervisorposition{Associate Professor}
%-------------------------------------------------------------------------------
% Co-Supervisor's Institute
% Command: \cosupinst
%\cosupervisorinstitute{BITS-Pilani, Hyderabad Campus}
%-------------------------------------------------------------------------------
% Your Examiner's name. Not currently used anywhere.
% Command: \examname
\examiner{}
%-------------------------------------------------------------------------------
% Name of your degree
% Command: \degreename
\degree{Ph.D. Research Scholar}
%-------------------------------------------------------------------------------
% The BITS Course Code for which this report is written
% COmmand: \ccode
\coursecode{\textbf{DOCTOR OF PHILOSOPHY}}
%\coursecode{BITS C799T}
%-------------------------------------------------------------------------------
% The name of the Course
% Command: \cname
\coursename{Thesis}
%-------------------------------------------------------------------------------
% Your name. Extend manually in case of multiple authors
% Command: \authornames
\authors{\textbf{Sneha Pradhan}}
%-------------------------------------------------------------------------------
% Your ID Number - used on the Title page and abstract
% Command: \idnum
\IDNumber{\textbf{2022PHXF0026H}}
%-------------------------------------------------------------------------------
% Your address
% Command: \addressnames
\addresses{}
%-------------------------------------------------------------------------------
% Your subject area
% Command: \subjectname
\subject{}
%-------------------------------------------------------------------------------
% Keywords for this report.
% Command: \keywordnames
\keywords{}
%-------------------------------------------------------------------------------
% University details
% Command: \univname
\university{\texorpdfstring{\href{http://www.bits-pilani.ac.in/} % URL
                {\textbf{Birla Institute of Technology and Science, Pilani}}} % University name
                {\textbf{Birla Institute of Technology and Science, Pilani}}}
%-------------------------------------------------------------------------------
% University details, in Capitals
% Command: \UNIVNAME
\UNIVERSITY{\texorpdfstring{\href{http://www.bits-pilani.ac.in/} % URL
                {\textbf{BIRLA INSTITUTE OF TECHNOLOGY AND SCIENCE, PILANI}}} % name in capitals
                {\textbf{BIRLA INSTITUTE OF TECHNOLOGY AND SCIENCE, PILANI}}}

%-------------------------------------------------------------------------------
% Campus Name
% Command: \campusname
%\campus{Hyderabad Campus}

%-------------------------------------------------------------------------------
% Campus Name, in capitals
% Command: \CAMPUSNAME
%\CAMPUS{HYDERABAD CAMPUS}


%-------------------------------------------------------------------------------
% Department Details
% Command: \deptname
\department{\texorpdfstring{\href{http://www.bits-pilani.ac.in/pilani/Mathematics/Mathematics} % Your department's URL
                {Mathematics}} % Your department's name
                {Mathematics}}
%-------------------------------------------------------------------------------
% Department details, in Capitals
% Command: \DEPTNAME
\DEPARTMENT{\texorpdfstring{\href{http://www.bits-pilani.ac.in/pilani/Mathematics/Mathematics} % Your department's URL
                {Mathematics}} % Your department's name in capitals
                {Mathematics}}
%-------------------------------------------------------------------------------
% Research Group Details
% Command: \groupname
\group{\texorpdfstring{\href{Research Group Web Site URL Here (include http://)}
                {Research Group Name}} % Your research group's name
                {Research Group Name}}
%-------------------------------------------------------------------------------
% Research Group Details, in Capitals
% Command: \GROUPNAME
\GROUP{\texorpdfstring{\href{Research Group Web Site URL Here (include http://)}
                {RESEARCH GROUP NAME (IN BLOCK CAPITALS)}}
                {RESEARCH GROUP NAME (IN BLOCK CAPITALS)}}
%-------------------------------------------------------------------------------
% Faculty details
% Command: \facname
\faculty{\texorpdfstring{\href{Faculty Web Site URL Here (include http://)}
                {Faculty Name}}
                {Faculty Name}}
%-------------------------------------------------------------------------------
% Faculty details, in Capitals
% Command: \FACNAME
\FACULTY{\texorpdfstring{\href{Faculty Web Site URL Here (include http://)}
                {FACULTY NAME (IN BLOCK CAPITALS)}}
                {FACULTY NAME (IN BLOCK CAPITALS)}}
%-------------------------------------------------------------------------------


